The AutoLyap software suite for computer-assisted Lyapunov analyses of first-order methods

We introduce AutoLyap, a software suite that assists with Lyapunov analyses of a wide class of first-order methods for structured optimization and inclusion problems. Lyapunov analyses are structured proof patterns, with historical roots in the study of dynamical systems, commonly used to establish convergence results for first-order methods. Building on previous work, the core idea behind AutoLyap is to recast the verification of the existence of a Lyapunov analysis as a semidefinite program (SDP), which can then be solved numerically using standard SDP solvers. Users of the package specify (i) the class of optimization or inclusion problems, (ii) the first-order method in question, and (iii) the type of Lyapunov analysis they wish to test. Once these inputs are provided, AutoLyap handles the SDP modeling and proceeds to solve the SDP numerically. We use the package to numerically verify and extend several convergence results. AutoLyap is currently available in Python and Julia.

==> data/linear_chambolle_pock/chambolle_pock_smooth_strongly_convex_tau_theta_rho.tex <==
tau,theta,rho
1.0,0.0,0.945854032988791
1.0084210526315789,0.0,0.9460719012713525
1.016842105263158,0.0,0.9463169926830233
1.0252631578947369,0.0,0.9465897604823112
1.0336842105263158,0.0,0.9468907199234309
1.0421052631578946,0.0,0.9472202975675827
1.0505263157894738,0.0,0.9475790871701975
1.0589473684210526,0.0,0.9479675590118859
1.0673684210526315,0.0,0.9483863115719942
1.0757894736842104,0.0,0.9488356970259701
1.0842105263157895,0.0,0.9493164292689471
1.0926315789473684,0.0,0.9498290792480475
1.1010526315789473,0.0,0.9503743984623725
1.1094736842105264,0.0,0.9509533040691167
1.1178947368421053,0.0,0.951566522648136
1.1263157894736842,0.0,0.9522146491781314
1.134736842105263,0.0,0.9528983825148316
1.1431578947368422,0.0,0.9536184082999171
1.151578947368421,0.0,0.954375385070307
1.16,0.0,0.9551700931024243
1.168421052631579,0.0,0.9560035152881028
1.176842105263158,0.0,0.9568760665870286
1.1852631578947368,0.0,0.957788654876822
1.1936842105263157,0.0,0.9587421128444475
1.2021052631578948,0.0,0.9597372485986853
1.2105263157894737,0.0,0.9607749283140947
1.2189473684210526,0.0,0.9618560131348204
1.2273684210526317,0.0,0.96298140673116
1.2357894736842105,0.0,0.9641520210625458
1.2442105263157894,0.0,0.9653687998161331
1.2526315789473683,0.0,0.9666327282466227
1.2610526315789474,0.0,0.9679447109811008
1.2694736842105263,0.0,0.9693060274439631
1.2778947368421052,0.0,0.9707175474541145
1.2863157894736843,0.0,0.9721802919921174
1.2947368421052632,0.0,0.9736956078568255
1.303157894736842,0.0,0.9752644216014232
1.311578947368421,0.0,0.9768880677802372
1.32,0.0,0.9785676956489624
1.328421052631579,0.0,0.980304616072317
1.3368421052631578,0.0,0.9821001050304403
1.345263157894737,0.0,0.983955515609523
1.3536842105263158,0.0,0.985872209072113
1.3621052631578947,0.0,0.9878517029583236
1.3705263157894736,0.0,0.989895373579202
1.3789473684210527,0.0,0.9920048185176711
1.3873684210526316,0.0,0.9941815760648751
1.3957894736842105,0.0,0.9964273087844049
1.4042105263157896,0.0,0.9987436754163355
1.0,0.031914893617021274,0.9274690551628737
1.0084210526315789,0.031914893617021274,0.9273641109102755
1.016842105263158,0.031914893617021274,0.9272860139026307
1.0252631578947369,0.031914893617021274,0.9272353244386977
1.0336842105263158,0.031914893617021274,0.9272120296463982
1.0421052631578946,0.031914893617021274,0.9272165379688886
1.0505263157894738,0.031914893617021274,0.9272493084718008
1.0589473684210526,0.031914893617021274,0.9273107458566301
1.0673684210526315,0.031914893617021274,0.9274014244738282
1.0757894736842104,0.031914893617021274,0.9275214755771231
1.0842105263157895,0.031914893617021274,0.9276715276937466
1.0926315789473684,0.031914893617021274,0.9278522711028927
1.1010526315789473,0.031914893617021274,0.9280649870652269
1.1094736842105264,0.031914893617021274,0.9283104315327364
1.1178947368421053,0.031914893617021274,0.9285893598680559
1.1263157894736842,0.031914893617021274,0.9289022583816404
1.134736842105263,0.031914893617021274,0.92925000167088
1.1431578947368422,0.031914893617021274,0.9296334457158082
1.151578947368421,0.031914893617021274,0.9300529017864392
1.16,0.031914893617021274,0.9305090866973842
1.168421052631579,0.031914893617021274,0.9310034215495762
1.176842105263158,0.031914893617021274,0.9315359368847567
1.1852631578947368,0.031914893617021274,0.9321078499697251
1.1936842105263157,0.031914893617021274,0.932719826567336
1.2021052631578948,0.031914893617021274,0.9333730714306512
1.2105263157894737,0.031914893617021274,0.9340680572331621
1.2189473684210526,0.031914893617021274,0.9348058113519073
1.2273684210526317,0.031914893617021274,0.9355875120727433
1.2357894736842105,0.031914893617021274,0.9364139028120917
1.2442105263157894,0.031914893617021274,0.9372860561998095
1.2526315789473683,0.031914893617021274,0.9382050511912894
1.2610526315789474,0.031914893617021274,0.9391719508439564
1.2694736842105263,0.031914893617021274,0.9401878113658313
1.2778947368421052,0.031914893617021274,0.9412539110835496
1.2863157894736843,0.031914893617021274,0.9423714093572926
1.2947368421052632,0.031914893617021274,0.9435414661829782
1.303157894736842,0.031914893617021274,0.9447653516235732
1.311578947368421,0.031914893617021274,0.9460444596770685
1.32,0.031914893617021274,0.9473800740142906
1.328421052631579,0.031914893617021274,0.9487736788723851
1.3368421052631578,0.031914893617021274,0.950226648206808
1.345263157894737,0.031914893617021274,0.951740591584894
1.3536842105263158,0.031914893617021274,0.9533169703363455
1.3621052631578947,0.031914893617021274,0.9549574488537473
1.3705263157894736,0.031914893617021274,0.9566636220542932
1.3789473684210527,0.031914893617021274,0.9584374517135075
1.3873684210526316,0.031914893617021274,0.960280542433793
1.3957894736842105,0.031914893617021274,0.9621948346739373
1.4042105263157896,0.031914893617021274,0.9641822691783091
1.4126315789473685,0.031914893617021274,0.9662448456365382
1.4210526315789473,0.031914893617021274,0.968384735086147
1.4294736842105262,0.031914893617021274,0.9706040659793871
1.4378947368421051,0.031914893617021274,0.9729051375770723
1.4463157894736842,0.031914893617021274,0.9752902686523157
1.454736842105263,0.031914893617021274,0.9777620173690593
1.4631578947368422,0.031914893617021274,0.980322877629078
1.471578947368421,0.031914893617021274,0.9829755459004446
1.48,0.031914893617021274,0.9857228059081535
1.4884210526315789,0.031914893617021274,0.9885675907144105
1.4968421052631578,0.031914893617021274,0.9915128991688107
1.5052631578947369,0.031914893617021274,0.9945619106292725
1.5136842105263157,0.031914893617021274,0.9977180409123321
1.0,0.06382978723404255,0.9231736575884497
1.0084210526315789,0.06382978723404255,0.9225532283317079
1.016842105263158,0.06382978723404255,0.9219330574951528
1.0252631578947369,0.06382978723404255,0.9213134367028033
1.0336842105263158,0.06382978723404255,0.9206941317552264
1.0421052631578946,0.06382978723404255,0.920075277252181
1.0505263157894738,0.06382978723404255,0.9194568622151564
1.0589473684210526,0.06382978723404255,0.918838738638442
1.0673684210526315,0.06382978723404255,0.9182213568719817
1.0757894736842104,0.06382978723404255,0.9176039396515989
1.0842105263157895,0.06382978723404255,0.9169874485805849
1.0926315789473684,0.06382978723404255,0.9163710046195774
1.1010526315789473,0.06382978723404255,0.9157553917038967
1.1094736842105264,0.06382978723404255,0.9151399731645142
1.1178947368421053,0.06382978723404255,0.9145247181240848
1.1263157894736842,0.06382978723404255,0.9139735273174665
1.134736842105263,0.06382978723404255,0.9135364890098572
1.1431578947368422,0.06382978723404255,0.9131937023485079
1.151578947368421,0.06382978723404255,0.9129317980259657
1.16,0.06382978723404255,0.9127441453456413
1.168421052631579,0.06382978723404255,0.9126250429653737
1.176842105263158,0.06382978723404255,0.9125702446290234
1.1852631578947368,0.06382978723404255,0.9125765207863878
1.1936842105263157,0.06382978723404255,0.9126417032930476
1.2021052631578948,0.06382978723404255,0.9127642912881129
1.2105263157894737,0.06382978723404255,0.9129426868130395
1.2189473684210526,0.06382978723404255,0.9131762144470486
1.2273684210526317,0.06382978723404255,0.9134644214509535
1.2357894736842105,0.06382978723404255,0.9138069078289845
1.2442105263157894,0.06382978723404255,0.9142041299337507
1.2526315789473683,0.06382978723404255,0.9146558527418165
1.2610526315789474,0.06382978723404255,0.9151624974911101
1.2694736842105263,0.06382978723404255,0.9157247469520371
1.2778947368421052,0.06382978723404255,0.9163430486541984
1.2863157894736843,0.06382978723404255,0.9170182333928096
1.2947368421052632,0.06382978723404255,0.9177510738300043
1.303157894736842,0.06382978723404255,0.9185428062055507
1.311578947368421,0.06382978723404255,0.919394135416951
1.32,0.06382978723404255,0.9203065969059026
1.328421052631579,0.06382978723404255,0.9212811647657873
1.3368421052631578,0.06382978723404255,0.9223193346397238
1.345263157894737,0.06382978723404255,0.9234225192349186
1.3536842105263158,0.06382978723404255,0.9245922420195711
1.3621052631578947,0.06382978723404255,0.9258301535137434
1.3705263157894736,0.06382978723404255,0.9271379699803219
1.3789473684210527,0.06382978723404255,0.9285174012184143
1.3873684210526316,0.06382978723404255,0.9299707585005308
1.3957894736842105,0.06382978723404255,0.9314994812011719
1.4042105263157896,0.06382978723404255,0.9331063548488601
1.4126315789473685,0.06382978723404255,0.9347930252552032
1.4210526315789473,0.06382978723404255,0.9365622121258639
1.4294736842105262,0.06382978723404255,0.9384161829657387
1.4378947368421051,0.06382978723404255,0.9403576508893821
1.4463157894736842,0.06382978723404255,0.9423892808690653
1.454736842105263,0.06382978723404255,0.9445139765748536
1.4631578947368422,0.06382978723404255,0.9467346959208953
1.471578947368421,0.06382978723404255,0.9490546455936055
1.48,0.06382978723404255,0.9514771237754758
1.4884210526315789,0.06382978723404255,0.9540056129844743
1.4968421052631578,0.06382978723404255,0.9566438546926292
1.5052631578947369,0.06382978723404255,0.9593956473700018
1.5136842105263157,0.06382978723404255,0.9622650770670589
1.5221052631578948,0.06382978723404255,0.9652564469752178
1.5305263157894737,0.06382978723404255,0.9683742601619088
1.5389473684210526,0.06382978723404255,0.9716233098906741
1.5473684210526315,0.06382978723404255,0.9750086094181825
1.5557894736842104,0.06382978723404255,0.9785354777750399
1.5642105263157895,0.06382978723404255,0.9822095310919394
1.5726315789473684,0.06382978723404255,0.9860367171841062
1.5810526315789475,0.06382978723404255,0.9900233213193133
1.5894736842105264,0.06382978723404255,0.994176000825064
1.5978947368421053,0.06382978723404255,0.9985018223878797
1.0,0.09574468085106383,0.9232226680878739
1.0084210526315789,0.09574468085106383,0.9226030141571755
1.016842105263158,0.09574468085106383,0.9219837449527404
1.0252631578947369,0.09574468085106383,0.9213649036873903
1.0336842105263158,0.09574468085106383,0.9207464044729932
1.0421052631578946,0.09574468085106383,0.920128412169106
1.0505263157894738,0.09574468085106383,0.9195106010874952
1.0589473684210526,0.09574468085106383,0.9188933330588043
1.0673684210526315,0.09574468085106383,0.9182768752789343
1.0757894736842104,0.09574468085106383,0.9176607206754852
1.0842105263157895,0.09574468085106383,0.9170443834373145
1.0926315789473684,0.09574468085106383,0.9164292453770031
1.1010526315789473,0.09574468085106383,0.9158145338305985
1.1094736842105264,0.09574468085106383,0.9151999677433196
1.1178947368421053,0.09574468085106383,0.9145851135253906
1.1263157894736842,0.09574468085106383,0.9139721532574185
1.134736842105263,0.09574468085106383,0.9133588436707214
1.1431578947368422,0.09574468085106383,0.9127460729805534
1.151578947368421,0.09574468085106383,0.9121335879463004
1.16,0.09574468085106383,0.9115216276768479
1.168421052631579,0.09574468085106383,0.9109101631156591
1.176842105263158,0.09574468085106383,0.910299049488458
1.1852631578947368,0.09574468085106383,0.9096882324338367
1.1936842105263157,0.09574468085106383,0.9090780811839068
1.2021052631578948,0.09574468085106383,0.9084682452230481
1.2105263157894737,0.09574468085106383,0.9078588186530396
1.2189473684210526,0.09574468085106383,0.9072498720561271
1.2273684210526317,0.09574468085106383,0.9066413641021427
1.2357894736842105,0.09574468085106383,0.9060330390930176
1.2442105263157894,0.09574468085106383,0.9054254206412224
1.2526315789473683,0.09574468085106383,0.9048181924936216
1.2610526315789474,0.09574468085106383,0.9042112659190025
1.2694736842105263,0.09574468085106383,0.9036047011613846
1.2778947368421052,0.09574468085106383,0.9029988494758072
1.2863157894736843,0.09574468085106383,0.9023930877447128
1.2947368421052632,0.09574468085106383,0.9018004759918767
1.303157894736842,0.09574468085106383,0.9013869802047338
1.311578947368421,0.09574468085106383,0.9011691239738866
1.32,0.09574468085106383,0.9011143456018544
1.328421052631579,0.09574468085106383,0.9012014804184219
1.3368421052631578,0.09574468085106383,0.9014161151426379
1.345263157894737,0.09574468085106383,0.9017482995986938
1.3536842105263158,0.09574468085106383,0.9021910121591645
1.3621052631578947,0.09574468085106383,0.9027393294954891
1.3705263157894736,0.09574468085106383,0.903389901313858
1.3789473684210527,0.09574468085106383,0.9041405246598515
1.3873684210526316,0.09574468085106383,0.904989964982633
1.3957894736842105,0.09574468085106383,0.9059377159846917
1.4042105263157896,0.09574468085106383,0.9069838523864746
1.4126315789473685,0.09574468085106383,0.9081289768218994
1.4210526315789473,0.09574468085106383,0.9093743634848579
1.4294736842105262,0.09574468085106383,0.9107211232185364
1.4378947368421051,0.09574468085106383,0.9121715476903773
1.4463157894736842,0.09574468085106383,0.913727343075152
1.454736842105263,0.09574468085106383,0.915391580438154
1.4631578947368422,0.09574468085106383,0.917166641546828
1.471578947368421,0.09574468085106383,0.9190558230748138
1.48,0.09574468085106383,0.9210626049989514
1.4884210526315789,0.09574468085106383,0.9231906969789634
1.4968421052631578,0.09574468085106383,0.9254442341589311
1.5052631578947369,0.09574468085106383,0.9278276261611609
1.5136842105263157,0.09574468085106383,0.9303456101943084
1.5221052631578948,0.09574468085106383,0.9330033065170937
1.5305263157894737,0.09574468085106383,0.9358061551611172
1.5389473684210526,0.09574468085106383,0.938760161531718
1.5473684210526315,0.09574468085106383,0.9418715240908568
1.5557894736842104,0.09574468085106383,0.9451470458952826
1.5642105263157895,0.09574468085106383,0.9485939742162373
1.5726315789473684,0.09574468085106383,0.9522200226183486
1.5810526315789475,0.09574468085106383,0.9560336470531183
1.5894736842105264,0.09574468085106383,0.9600436761820674
1.5978947368421053,0.09574468085106383,0.964259722953102
1.6063157894736841,0.09574468085106383,0.9686921110569529
1.614736842105263,0.09574468085106383,0.9733518362045288
1.6231578947368421,0.09574468085106383,0.9782510480345081
1.631578947368421,0.09574468085106383,0.983402408773145
1.6400000000000001,0.09574468085106383,0.988819858410352
1.648421052631579,0.09574468085106383,0.9945184068283197
1.0,0.1276595744680851,0.9232716651031296
1.0084210526315789,0.1276595744680851,0.9226527959708619
1.016842105263158,0.1276595744680851,0.9220341738500792
1.0252631578947369,0.1276595744680851,0.9214162370853956
1.0336842105263158,0.1276595744680851,0.9207985796356297
1.0421052631578946,0.1276595744680851,0.9201812499086373
1.0505263157894738,0.1276595744680851,0.9195646627777023
1.0589473684210526,0.1276595744680851,0.9189483588479561
1.0673684210526315,0.1276595744680851,0.918332581478353
1.0757894736842104,0.1276595744680851,0.9177169799759213
1.0842105263157895,0.1276595744680851,0.9171018003253266
1.0926315789473684,0.1276595744680851,0.9164873654372059
1.1010526315789473,0.1276595744680851,0.9158734738084604
1.1094736842105264,0.1276595744680851,0.9152599130857197
1.1178947368421053,0.1276595744680851,0.9146465946541866
1.1263157894736842,0.1276595744680851,0.9140338441238782
1.134736842105263,0.1276595744680851,0.9134215101494192
1.1431578947368422,0.1276595744680851,0.9128096404065218
1.151578947368421,0.1276595744680851,0.912198073892796
1.16,0.1276595744680851,0.9115868737917481
1.168421052631579,0.1276595744680851,0.9109762158404919
1.176842105263158,0.1276595744680851,0.910366050869925
1.1852631578947368,0.1276595744680851,0.909756465330247
1.1936842105263157,0.1276595744680851,0.9091472112822885
1.2021052631578948,0.1276595744680851,0.9085383146930326
1.2105263157894737,0.1276595744680851,0.907929938444795
1.2189473684210526,0.1276595744680851,0.9073217956738517
1.2273684210526317,0.1276595744680851,0.9067142836292987
1.2357894736842105,0.1276595744680851,0.9061069408344338
1.2442105263157894,0.1276595744680851,0.905500431580549
1.2526315789473683,0.1276595744680851,0.904894123743361
1.2610526315789474,0.1276595744680851,0.9042880497872829
1.2694736842105263,0.1276595744680851,0.9036826784722507
1.2778947368421052,0.1276595744680851,0.9030779007034653
1.2863157894736843,0.1276595744680851,0.902473200066197
1.2947368421052632,0.1276595744680851,0.9018690576185691
1.303157894736842,0.1276595744680851,0.9012654085181566
1.311578947368421,0.1276595744680851,0.9006620645486692
1.32,0.1276595744680851,0.9000592150478042
1.328421052631579,0.1276595744680851,0.8994568585749221
1.3368421052631578,0.1276595744680851,0.8988548058550805
1.345263157894737,0.1276595744680851,0.8982533812550173
1.3536842105263158,0.1276595744680851,0.8976521323920679
1.3621052631578947,0.1276595744680851,0.897051215171814
1.3705263157894736,0.1276595744680851,0.8964509963952878
1.3789473684210527,0.1276595744680851,0.8958512892704675
1.3873684210526316,0.1276595744680851,0.8952519018803287
1.3957894736842105,0.1276595744680851,0.8946527833904838
1.4042105263157896,0.1276595744680851,0.8940541696283617
1.4126315789473685,0.1276595744680851,0.8934559213812463
1.4210526315789473,0.1276595744680851,0.8928585076355375
1.4294736842105262,0.1276595744680851,0.8925026028782668
1.4378947368421051,0.1276595744680851,0.892532959484015
1.4463157894736842,0.1276595744680851,0.8928655387398976
1.454736842105263,0.1276595744680851,0.8934520590928514
1.4631578947368422,0.1276595744680851,0.8942630159881446
1.471578947368421,0.1276595744680851,0.8952796884968848
1.48,0.1276595744680851,0.8964903056621552
1.4884210526315789,0.1276595744680851,0.8978878083289601
1.4968421052631578,0.1276595744680851,0.8994682825141354
1.5052631578947369,0.1276595744680851,0.9012304404386668
1.5136842105263157,0.1276595744680851,0.9031749477107951
1.5221052631578948,0.1276595744680851,0.9053040897688334
1.5305263157894737,0.1276595744680851,0.9076214543601964
1.5389473684210526,0.1276595744680851,0.9101320076579213
1.5473684210526315,0.1276595744680851,0.9128417740575969
1.5557894736842104,0.1276595744680851,0.9157579370039457
1.5642105263157895,0.1276595744680851,0.918888714923014
1.5726315789473684,0.1276595744680851,0.9222434863941089
1.5810526315789475,0.1276595744680851,0.9258327027146152
1.5894736842105264,0.1276595744680851,0.9296680651614224
1.5978947368421053,0.1276595744680851,0.9337624833115115
1.6063157894736841,0.1276595744680851,0.9381302447663984
1.614736842105263,0.1276595744680851,0.9427871112884532
1.6231578947368421,0.1276595744680851,0.9477504202222917
1.631578947368421,0.1276595744680851,0.9530393374516279
1.6400000000000001,0.1276595744680851,0.9586749076515844
1.648421052631579,0.1276595744680851,0.9646804295471156
1.656842105263158,0.1276595744680851,0.9710815805128732
1.6652631578947368,0.1276595744680851,0.9779068233092403
1.6736842105263157,0.1276595744680851,0.9851876819084282
1.6821052631578948,0.1276595744680851,0.99295924407852
1.0,0.15957446808510636,0.9233205570371865
1.0084210526315789,0.15957446808510636,0.922702378453323
1.016842105263158,0.15957446808510636,0.9220847722253893
1.0252631578947369,0.15957446808510636,0.921467554569972
1.0336842105263158,0.15957446808510636,0.9208507816556448
1.0421052631578946,0.15957446808510636,0.9202344127161268
1.0505263157894738,0.15957446808510636,0.9196184934089615
1.0589473684210526,0.15957446808510636,0.9190030162862968
1.0673684210526315,0.15957446808510636,0.9183880071768726
1.0757894736842104,0.15957446808510636,0.9177734813220013
1.0842105263157895,0.15957446808510636,0.9171594424251452
1.0926315789473684,0.15957446808510636,0.9165452718734741
1.1010526315789473,0.15957446808510636,0.9159322378654906
1.1094736842105264,0.15957446808510636,0.9153193086312967
1.1178947368421053,0.15957446808510636,0.9147071624029195
1.1263157894736842,0.15957446808510636,0.914095516265661
1.134736842105263,0.15957446808510636,0.9134840186989095
1.1431578947368422,0.15957446808510636,0.9128727910574526
1.151578947368421,0.15957446808510636,0.912261962890625
1.16,0.15957446808510636,0.9116523874436098
1.168421052631579,0.15957446808510636,0.9110422134344844
1.176842105263158,0.15957446808510636,0.9104330539703369
1.1852631578947368,0.15957446808510636,0.9098246071225731
1.1936842105263157,0.15957446808510636,0.9092162098495464
1.2021052631578948,0.15957446808510636,0.9086082241265103
1.2105263157894737,0.15957446808510636,0.9080007533739263
1.2189473684210526,0.15957446808510636,0.9073938137535151
1.2273684210526317,0.15957446808510636,0.9067871883762564
1.2357894736842105,0.15957446808510636,0.9061809413806259
1.2442105263157894,0.15957446808510636,0.9055752940503226
1.2526315789473683,0.15957446808510636,0.9049698965436619
1.2610526315789474,0.15957446808510636,0.904365068651714
1.2694736842105263,0.15957446808510636,0.9037605810954119
1.2778947368421052,0.15957446808510636,0.9031566420680974
1.2863157894736843,0.15957446808510636,0.9025530913813782
1.2947368421052632,0.15957446808510636,0.9019499620771967
1.303157894736842,0.15957446808510636,0.9013472639417159
1.311578947368421,0.15957446808510636,0.9007450792969394
1.32,0.15957446808510636,0.9001432314653357
1.328421052631579,0.15957446808510636,0.8995416124744224
1.3368421052631578,0.15957446808510636,0.8989408610914325
1.345263157894737,0.15957446808510636,0.8983402242265583
1.3536842105263158,0.15957446808510636,0.8977403487097035
1.3621052631578947,0.15957446808510636,0.8971405625343323
1.3705263157894736,0.15957446808510636,0.8965414487784074
1.3789473684210527,0.15957446808510636,0.8959425650537014
1.3873684210526316,0.15957446808510636,0.8953442912052196
1.3957894736842105,0.15957446808510636,0.8947462439537048
1.4042105263157896,0.15957446808510636,0.8941489392900621
1.4126315789473685,0.15957446808510636,0.8935518573280206
1.4210526315789473,0.15957446808510636,0.8929551528708544
1.4294736842105262,0.15957446808510636,0.8923590338172289
1.4378947368421051,0.15957446808510636,0.8917632100510673
1.4463157894736842,0.15957446808510636,0.8911678741578726
1.454736842105263,0.15957446808510636,0.8905728903300769
1.4631578947368422,0.15957446808510636,0.8899785009052721
1.471578947368421,0.15957446808510636,0.8893844385993361
1.48,0.15957446808510636,0.8887907196722153
1.4884210526315789,0.15957446808510636,0.8881975668473387
1.4968421052631578,0.15957446808510636,0.8876048855026966
1.5052631578947369,0.15957446808510636,0.8870125680705314
1.5136842105263157,0.15957446808510636,0.8864326240673108
1.5221052631578948,0.15957446808510636,0.8864503726363182
1.5305263157894737,0.15957446808510636,0.8871609202788022
1.5389473684210526,0.15957446808510636,0.8883911442244425
1.5473684210526315,0.15957446808510636,0.8900560900783603
1.5557894736842104,0.15957446808510636,0.8921107724900139
1.5642105263157895,0.15957446808510636,0.894531865839781
1.5726315789473684,0.15957446808510636,0.8973092312071458
1.5810526315789475,0.15957446808510636,0.9004417205578648
1.5894736842105264,0.15957446808510636,0.9039347347725197
1.5978947368421053,0.15957446808510636,0.9077990500336455
1.6063157894736841,0.15957446808510636,0.9120501074648928
1.614736842105263,0.15957446808510636,0.9167076614276084
1.6231578947368421,0.15957446808510636,0.9217957276869129
1.631578947368421,0.15957446808510636,0.9273427520247424
1.6400000000000001,0.15957446808510636,0.9333818647282897
1.648421052631579,0.15957446808510636,0.9399513849084542
1.656842105263158,0.15957446808510636,0.9470953295449362
1.6652631578947368,0.15957446808510636,0.9548643128855474
1.6736842105263157,0.15957446808510636,0.9633165090344846
1.6821052631578948,0.15957446808510636,0.97251889522704
1.6905263157894737,0.15957446808510636,0.982548811282868
1.6989473684210528,0.15957446808510636,0.993495943027483
1.0,0.19148936170212766,0.9233694090553399
1.0084210526315789,0.19148936170212766,0.9227520423555688
1.016842105263158,0.19148936170212766,0.9221351118176244
1.0252631578947369,0.19148936170212766,0.9215185632929206
1.0336842105263158,0.19148936170212766,0.9209027578972382
1.0421052631578946,0.19148936170212766,0.9202873456988527
1.0505263157894738,0.19148936170212766,0.9196722631031662
1.0589473684210526,0.19148936170212766,0.9190576369092014
1.0673684210526315,0.19148936170212766,0.9184435159131681
1.0757894736842104,0.19148936170212766,0.9178297759990528
1.0842105263157895,0.19148936170212766,0.9172161816859443
1.0926315789473684,0.19148936170212766,0.916603472083807
1.1010526315789473,0.19148936170212766,0.9159914209585622
1.1094736842105264,0.19148936170212766,0.9153795503088986
1.1178947368421053,0.19148936170212766,0.9147680492296786
1.1263157894736842,0.19148936170212766,0.9141570806177697
1.134736842105263,0.19148936170212766,0.9135465362642208
1.1431578947368422,0.19148936170212766,0.9129362701060018
1.151578947368421,0.19148936170212766,0.9123267264767492
1.16,0.19148936170212766,0.9117175499786754
1.168421052631579,0.19148936170212766,0.9111087586834401
1.176842105263158,0.19148936170212766,0.9105004474777161
1.1852631578947368,0.19148936170212766,0.9098924025865927
1.1936842105263157,0.19148936170212766,0.9092845916748047
1.2021052631578948,0.19148936170212766,0.9086782336262331
1.2105263157894737,0.19148936170212766,0.9080715458840132
1.2189473684210526,0.19148936170212766,0.9074655848107795
1.2273684210526317,0.19148936170212766,0.9068593978736317
1.2357894736842105,0.19148936170212766,0.9062546923041737
1.2442105263157894,0.19148936170212766,0.9056499395283026
1.2526315789473683,0.19148936170212766,0.9050457477651435
1.2610526315789474,0.19148936170212766,0.9044417739614801
1.2694736842105263,0.19148936170212766,0.9038381427380955
1.2778947368421052,0.19148936170212766,0.9032353346547097
1.2863157894736843,0.19148936170212766,0.9026325941013056
1.2947368421052632,0.19148936170212766,0.9020306995225837
1.303157894736842,0.19148936170212766,0.9014286398814875
1.311578947368421,0.19148936170212766,0.9008277768280095
1.32,0.19148936170212766,0.9002270411456266
1.328421052631579,0.19148936170212766,0.8996267337361132
1.3368421052631578,0.19148936170212766,0.8990268000061405
1.345263157894737,0.19148936170212766,0.898427370938407
1.3536842105263158,0.19148936170212766,0.8978282711223073
1.3621052631578947,0.19148936170212766,0.8972297161826646
1.3705263157894736,0.19148936170212766,0.8966312408447266
1.3789473684210527,0.19148936170212766,0.8960338590622996
1.3873684210526316,0.19148936170212766,0.895436522446289
1.3957894736842105,0.19148936170212766,0.8948397358071816
1.4042105263157896,0.19148936170212766,0.8942432701260259
1.4126315789473685,0.19148936170212766,0.89364743232818
1.4210526315789473,0.19148936170212766,0.8930518021807075
1.4294736842105262,0.19148936170212766,0.8924567718086109
1.4378947368421051,0.19148936170212766,0.8918621000248095
1.4463157894736842,0.19148936170212766,0.8912678053602576
1.454736842105263,0.19148936170212766,0.8906741201990371
1.4631578947368422,0.19148936170212766,0.8900807052768869
1.471578947368421,0.19148936170212766,0.8894878242763298
1.48,0.19148936170212766,0.888895258307457
1.4884210526315789,0.19148936170212766,0.8883032789417484
1.4968421052631578,0.19148936170212766,0.8877117454849213
1.5052631578947369,0.19148936170212766,0.8871205353407277
1.5136842105263157,0.19148936170212766,0.8865298261598582
1.5221052631578948,0.19148936170212766,0.8859394555620383
1.5305263157894737,0.19148936170212766,0.8853496029096277
1.5389473684210526,0.19148936170212766,0.8847601658826534
1.5473684210526315,0.19148936170212766,0.8841711431286967
1.5557894736842104,0.19148936170212766,0.8835824709385633
1.5642105263157895,0.19148936170212766,0.8829943675837058
1.5726315789473684,0.19148936170212766,0.882423713163007
1.5810526315789475,0.19148936170212766,0.8830797605542102
1.5894736842105264,0.19148936170212766,0.8850716804317926
1.5978947368421053,0.19148936170212766,0.888011448436373
1.6063157894736841,0.19148936170212766,0.8917538597024759
1.614736842105263,0.19148936170212766,0.8962454632655863
1.6231578947368421,0.19148936170212766,0.9014791250219787
1.631578947368421,0.19148936170212766,0.9074769603312234
1.6400000000000001,0.19148936170212766,0.9142829278689533
1.648421052631579,0.19148936170212766,0.9219605545476952
1.656842105263158,0.19148936170212766,0.9305927566601895
1.6652631578947368,0.19148936170212766,0.9402835335149575
1.6736842105263157,0.19148936170212766,0.9511611461639404
1.6821052631578948,0.19148936170212766,0.9633832576755594
1.6905263157894737,0.19148936170212766,0.9771433658906972
1.6989473684210528,0.19148936170212766,0.9926809427397529
1.0,0.22340425531914893,0.9234180439962074
1.0084210526315789,0.22340425531914893,0.9228016216893593
1.016842105263158,0.22340425531914893,0.9221855700079686
1.0252631578947369,0.22340425531914893,0.9215698828911627
1.0336842105263158,0.22340425531914893,0.9209548228773201
1.0421052631578946,0.22340425531914893,0.9203401243394183
1.0505263157894738,0.22340425531914893,0.91972589073157
1.0589473684210526,0.22340425531914893,0.9191118151502451
1.0673684210526315,0.22340425531914893,0.9184987482149154
1.0757894736842104,0.22340425531914893,0.9178855400496104
1.0842105263157895,0.22340425531914893,0.9172736252185132
1.0926315789473684,0.22340425531914893,0.9166616191723733
1.1010526315789473,0.22340425531914893,0.9160502270451616
1.1094736842105264,0.22340425531914893,0.9154392044920314
1.1178947368421053,0.22340425531914893,0.9148283898821319
1.1263157894736842,0.22340425531914893,0.9142185239961691
1.134736842105263,0.22340425531914893,0.9136089310404714
1.1431578947368422,0.22340425531914893,0.9129997234613256
1.151578947368421,0.22340425531914893,0.9123908653709805
1.16,0.22340425531914893,0.9117826820775008
1.168421052631579,0.22340425531914893,0.9111747938477492
1.176842105263158,0.22340425531914893,0.9105670154094696
1.1852631578947368,0.22340425531914893,0.9099605237142896
1.1936842105263157,0.22340425531914893,0.9093539318928379
1.2021052631578948,0.22340425531914893,0.9087479320360217
1.2105263157894737,0.22340425531914893,0.9081422565504909
1.2189473684210526,0.22340425531914893,0.907537311318265
1.2273684210526317,0.22340425531914893,0.9069321155539001
1.2357894736842105,0.22340425531914893,0.9063283109362601
1.2442105263157894,0.22340425531914893,0.9057244740688475
1.2526315789473683,0.22340425531914893,0.9051210848265328
1.2610526315789474,0.22340425531914893,0.9045182657991973
1.2694736842105263,0.22340425531914893,0.9039158038458481
1.2778947368421052,0.22340425531914893,0.9033138049680929
1.2863157894736843,0.22340425531914893,0.902712283591427
1.2947368421052632,0.22340425531914893,0.902111105620861
1.303157894736842,0.22340425531914893,0.9015105243597645
1.311578947368421,0.22340425531914893,0.9009104073793424
1.32,0.22340425531914893,0.9003106569953161
1.328421052631579,0.22340425531914893,0.8997112501419906
1.3368421052631578,0.22340425531914893,0.8991117477416992
1.345263157894737,0.22340425531914893,0.8985140589220464
1.3536842105263158,0.22340425531914893,0.8979161049219329
1.3621052631578947,0.22340425531914893,0.8973185151990037
1.3705263157894736,0.22340425531914893,0.8967213607238591
1.3789473684210527,0.22340425531914893,0.8961248426394377
1.3873684210526316,0.22340425531914893,0.8955286676273317
1.3957894736842105,0.22340425531914893,0.8949328762901132
1.4042105263157896,0.22340425531914893,0.8943374119699001
1.4126315789473685,0.22340425531914893,0.8937425610783976
1.4210526315789473,0.22340425531914893,0.8931482732041331
1.4294736842105262,0.22340425531914893,0.8925544023522889
1.4378947368421051,0.22340425531914893,0.891960752194791
1.4463157894736842,0.22340425531914893,0.8913676639040204
1.454736842105263,0.22340425531914893,0.890775085005771
1.4631578947368422,0.22340425531914893,0.8901827891113498
1.471578947368421,0.22340425531914893,0.8895910355522574
1.48,0.22340425531914893,0.8889998048625785
1.4884210526315789,0.22340425531914893,0.888408787116532
1.4968421052631578,0.22340425531914893,0.8878182172775269
1.5052631578947369,0.22340425531914893,0.8872283090877318
1.5136842105263157,0.22340425531914893,0.8866387631651378
1.5221052631578948,0.22340425531914893,0.8860495686421928
1.5305263157894737,0.22340425531914893,0.885460972823239
1.5389473684210526,0.22340425531914893,0.8848726352443919
1.5473684210526315,0.22340425531914893,0.8842847696114404
1.5557894736842104,0.22340425531914893,0.8836974316573105
1.5642105263157895,0.22340425531914893,0.8831104953433169
1.5726315789473684,0.22340425531914893,0.8825239231118758
1.5810526315789475,0.22340425531914893,0.8819379103388201
1.5894736842105264,0.22340425531914893,0.8813522101727358
1.5978947368421053,0.22340425531914893,0.8807669430825626
1.6063157894736841,0.22340425531914893,0.880473257063386
1.614736842105263,0.22340425531914893,0.8833217718311062
1.6231578947368421,0.22340425531914893,0.8885004802186813
1.631578947368421,0.22340425531914893,0.8954470668832073
1.6400000000000001,0.22340425531914893,0.9040653703268617
1.648421052631579,0.22340425531914893,0.9144353121519089
1.656842105263158,0.22340425531914893,0.9267488859522928
1.6652631578947368,0.22340425531914893,0.941300651777965
1.6736842105263157,0.22340425531914893,0.9585032686291015
1.6821052631578948,0.22340425531914893,0.9789231023460161
1.0,0.2553191489361702,0.923466784660377
1.0084210526315789,0.2553191489361702,0.9228511455266926
1.016842105263158,0.2553191489361702,0.922235861234185
1.0252631578947369,0.2553191489361702,0.9216208438738249
1.0336842105263158,0.2553191489361702,0.9210068044494619
1.0421052631578946,0.2553191489361702,0.9203928778479167
1.0505263157894738,0.2553191489361702,0.9197795704631062
1.0589473684210526,0.2553191489361702,0.9191665944954366
1.0673684210526315,0.2553191489361702,0.9185538281853951
1.0757894736842104,0.2553191489361702,0.917942198036144
1.0842105263157895,0.2553191489361702,0.917330635579674
1.0926315789473684,0.2553191489361702,0.9167192503336992
1.1010526315789473,0.2553191489361702,0.9161089211665967
1.1094736842105264,0.2553191489361702,0.9154988139262059
1.1178947368421053,0.2553191489361702,0.9148890672404377
1.1263157894736842,0.2553191489361702,0.9142792224847653
1.134736842105263,0.2553191489361702,0.9136705397977494
1.1431578947368422,0.2553191489361702,0.9130628642806187
1.151578947368421,0.2553191489361702,0.9124550036112851
1.16,0.2553191489361702,0.9118476515332077
1.168421052631579,0.2553191489361702,0.91124063519419
1.176842105263158,0.2553191489361702,0.9106342496825164
1.1852631578947368,0.2553191489361702,0.9100281594783155
1.1936842105263157,0.2553191489361702,0.9094226671159049
1.2021052631578948,0.2553191489361702,0.9088175700808279
1.2105263157894737,0.2553191489361702,0.9082126526445791
1.2189473684210526,0.2553191489361702,0.9076085090628112
1.2273684210526317,0.2553191489361702,0.9070050736163466
1.2357894736842105,0.2553191489361702,0.9064017775854154
1.2442105263157894,0.2553191489361702,0.9057989893208287
1.2526315789473683,0.2553191489361702,0.9051960706710815
1.2610526315789474,0.2553191489361702,0.9045946449041367
1.2694736842105263,0.2553191489361702,0.9039932627201779
1.2778947368421052,0.2553191489361702,0.9033918976674613
1.2863157894736843,0.2553191489361702,0.9027917421890379
1.2947368421052632,0.2553191489361702,0.902191162109375
1.303157894736842,0.2553191489361702,0.9015919932699035
1.311578947368421,0.2553191489361702,0.9009928713658155
1.32,0.2553191489361702,0.9003941029859561
1.328421052631579,0.2553191489361702,0.8997958581812782
1.3368421052631578,0.2553191489361702,0.8991980346136188
1.345263157894737,0.2553191489361702,0.8986007282592254
1.3536842105263158,0.2553191489361702,0.8980037190340227
1.3621052631578947,0.2553191489361702,0.8974073277868229
1.3705263157894736,0.2553191489361702,0.8968111276626587
1.3789473684210527,0.2553191489361702,0.896215707311967
1.3873684210526316,0.2553191489361702,0.8956205919485001
1.3957894736842105,0.2553191489361702,0.8950252532958984
1.4042105263157896,0.2553191489361702,0.894431583583355
1.4126315789473685,0.2553191489361702,0.8938379250475919
1.4210526315789473,0.2553191489361702,0.8932442665100098
1.4294736842105262,0.2553191489361702,0.8926517236996006
1.4378947368421051,0.2553191489361702,0.8920590578345582
1.4463157894736842,0.2553191489361702,0.8914672278915532
1.454736842105263,0.2553191489361702,0.8908757597700969
1.4631578947368422,0.2553191489361702,0.8902847471335917
1.471578947368421,0.2553191489361702,0.8896940013455605
1.48,0.2553191489361702,0.8891038447627579
1.4884210526315789,0.2553191489361702,0.8885140319907805
1.4968421052631578,0.2553191489361702,0.8879246692813467
1.5052631578947369,0.2553191489361702,0.8873359412109494
1.5136842105263157,0.2553191489361702,0.886747472954994
1.5221052631578948,0.2553191489361702,0.8861594197514933
1.5305263157894737,0.2553191489361702,0.8855719493558354
1.5389473684210526,0.2553191489361702,0.8849848434292653
1.5473684210526315,0.2553191489361702,0.88439829647632
1.5557894736842104,0.2553191489361702,0.8838119506826843
1.5642105263157895,0.2553191489361702,0.8832262818932577
1.5726315789473684,0.2553191489361702,0.8826410183746702
1.5810526315789475,0.2553191489361702,0.8820561184902544
1.5894736842105264,0.2553191489361702,0.8814716972738097
1.5978947368421053,0.2553191489361702,0.8808876753419099
1.6063157894736841,0.2553191489361702,0.8803041337587274
1.614736842105263,0.2553191489361702,0.8798099452169481
1.6231578947368421,0.2553191489361702,0.8856205352067263
1.631578947368421,0.2553191489361702,0.896698032972381
1.6400000000000001,0.2553191489361702,0.9119249359446258
1.648421052631579,0.2553191489361702,0.9317431050112646
1.656842105263158,0.2553191489361702,0.9572953653696459
1.6652631578947368,0.2553191489361702,0.9905512088444084
1.0,0.28723404255319146,0.9235153198242188
1.0084210526315789,0.28723404255319146,0.9229004920616717
1.016842105263158,0.28723404255319146,0.9222860326990485
1.0252631578947369,0.28723404255319146,0.9216721076354588
1.0336842105263158,0.28723404255319146,0.9210586846465958
1.0421052631578946,0.28723404255319146,0.920445381605532
1.0505263157894738,0.28723404255319146,0.9198322296142578
1.0589473684210526,0.28723404255319146,0.9192209196880867
1.0673684210526315,0.28723404255319146,0.9186091402934835
1.0757894736842104,0.28723404255319146,0.9179978052561637
1.0842105263157895,0.28723404255319146,0.9173874556727242
1.0926315789473684,0.28723404255319146,0.9167773725939696
1.1010526315789473,0.28723404255319146,0.9161674361675978
1.1094736842105264,0.28723404255319146,0.9155582984722059
1.1178947368421053,0.28723404255319146,0.9149495763713276
1.1263157894736842,0.28723404255319146,0.9143412123366943
1.134736842105263,0.28723404255319146,0.9137330045778072
1.1431578947368422,0.28723404255319146,0.9131257225526497
1.151578947368421,0.28723404255319146,0.91251858835858
1.16,0.28723404255319146,0.9119124335693414
1.168421052631579,0.28723404255319146,0.9113064909670356
1.176842105263158,0.28723404255319146,0.9107009453873616
1.1852631578947368,0.28723404255319146,0.9100958098024421
1.1936842105263157,0.28723404255319146,0.9094912561331512
1.2021052631578948,0.28723404255319146,0.9088869094839538
1.2105263157894737,0.28723404255319146,0.9082834422888482
1.2189473684210526,0.28723404255319146,0.9076801611727205
1.2273684210526317,0.28723404255319146,0.9070774303236249
1.2357894736842105,0.28723404255319146,0.9064749479148304
1.2442105263157894,0.28723404255319146,0.9058731791446917
1.2526315789473683,0.28723404255319146,0.9052720079498613
1.2610526315789474,0.28723404255319146,0.9046709385584109
1.2694736842105263,0.28723404255319146,0.9040701910853386
1.2778947368421052,0.28723404255319146,0.9034706358806943
1.2863157894736843,0.28723404255319146,0.9028710089114611
1.2947368421052632,0.28723404255319146,0.902271805323835
1.303157894736842,0.28723404255319146,0.9016731902956963
1.311578947368421,0.28723404255319146,0.9010751247406006
1.32,0.28723404255319146,0.9004774394625201
1.328421052631579,0.28723404255319146,0.8998802900323426
1.3368421052631578,0.28723404255319146,0.8992833492811769
1.345263157894737,0.28723404255319146,0.8986871398719813
1.3536842105263158,0.28723404255319146,0.8980912491715571
1.3621052631578947,0.28723404255319146,0.8974958323042301
1.3705263157894736,0.28723404255319146,0.8969008545727775
1.3789473684210527,0.28723404255319146,0.8963060376681824
1.3873684210526316,0.28723404255319146,0.8957123234895334
1.3957894736842105,0.28723404255319146,0.8951186686217625
1.4042105263157896,0.28723404255319146,0.8945255969474601
1.4126315789473685,0.28723404255319146,0.8939328193664551
1.4210526315789473,0.28723404255319146,0.8933407077574884
1.4294736842105262,0.28723404255319146,0.892748871186086
1.4378947368421051,0.28723404255319146,0.8921575644380937
1.4463157894736842,0.28723404255319146,0.8915666912262168
1.454736842105263,0.28723404255319146,0.8909760704264045
1.4631578947368422,0.28723404255319146,0.8903862737479358
1.471578947368421,0.28723404255319146,0.8897967710490775
1.48,0.28723404255319146,0.8892077582577258
1.4884210526315789,0.28723404255319146,0.8886191854862773
1.4968421052631578,0.28723404255319146,0.8880309630967531
1.5052631578947369,0.28723404255319146,0.8874433080209201
1.5136842105263157,0.28723404255319146,0.8868560796045131
1.5221052631578948,0.28723404255319146,0.8862691733811516
1.5305263157894737,0.28723404255319146,0.8856828264861178
1.5389473684210526,0.28723404255319146,0.8850968480110168
1.5473684210526315,0.28723404255319146,0.8845114607647702
1.5557894736842104,0.28723404255319146,0.8839263913387185
1.5642105263157895,0.28723404255319146,0.883341863745045
1.5726315789473684,0.28723404255319146,0.8827578017026099
1.5810526315789475,0.28723404255319146,0.8821740485582268
1.5894736842105264,0.28723404255319146,0.8815908133983612
1.5978947368421053,0.28723404255319146,0.8810080915109211
1.6063157894736841,0.28723404255319146,0.8804257263909676
1.614736842105263,0.28723404255319146,0.8906232585040925
1.6231578947368421,0.28723404255319146,0.9151968955993652
1.631578947368421,0.28723404255319146,0.9528670450672507
1.0,0.3191489361702127,0.92356393258342
1.0084210526315789,0.3191489361702127,0.9229498346803666
1.016842105263158,0.3191489361702127,0.9223362543752955
1.0252631578947369,0.3191489361702127,0.9217230376953012
1.0336842105263158,0.3191489361702127,0.9211103925390489
1.0421052631578946,0.3191489361702127,0.9204980134209109
1.0505263157894738,0.3191489361702127,0.9198863506317139
1.0589473684210526,0.3191489361702127,0.9192752987737549
1.0673684210526315,0.3191489361702127,0.9186644315395824
1.0757894736842104,0.3191489361702127,0.9180536267813295
1.0842105263157895,0.3191489361702127,0.9174443345664258
1.0926315789473684,0.3191489361702127,0.9168348237872124
1.1010526315789473,0.3191489361702127,0.9162260288721882
1.1094736842105264,0.3191489361702127,0.9156178236089545
1.1178947368421053,0.3191489361702127,0.9150098081863689
1.1263157894736842,0.3191489361702127,0.9144021197716938
1.134736842105263,0.3191489361702127,0.9137954711923157
1.1431578947368422,0.3191489361702127,0.9131888445381264
1.151578947368421,0.3191489361702127,0.9125828516644106
1.16,0.3191489361702127,0.9119773041857115
1.168421052631579,0.3191489361702127,0.911372154878336
1.176842105263158,0.3191489361702127,0.9107675956029198
1.1852631578947368,0.3191489361702127,0.9101634165035648
1.1936842105263157,0.3191489361702127,0.9095597340883614
1.2021052631578948,0.3191489361702127,0.9089565313342973
1.2105263157894737,0.3191489361702127,0.9083532094919065
1.2189473684210526,0.3191489361702127,0.9077510833740234
1.2273684210526317,0.3191489361702127,0.9071496856613521
1.2357894736842105,0.3191489361702127,0.9065483883359775
1.2442105263157894,0.3191489361702127,0.9059475220428794
1.2526315789473683,0.3191489361702127,0.9053471107336009
1.2610526315789474,0.3191489361702127,0.9047467708587646
1.2694736842105263,0.3191489361702127,0.9041476787015199
1.2778947368421052,0.3191489361702127,0.9035486243519699
1.2863157894736843,0.3191489361702127,0.9029501366576369
1.2947368421052632,0.3191489361702127,0.9023520200207713
1.303157894736842,0.3191489361702127,0.90175436809659
1.311578947368421,0.3191489361702127,0.9011572413110116
1.32,0.3191489361702127,0.9005606176069705
1.328421052631579,0.3191489361702127,0.8999644131436071
1.3368421052631578,0.3191489361702127,0.8993686414669355
1.345263157894737,0.3191489361702127,0.8987734618140166
1.3536842105263158,0.3191489361702127,0.8981785363166637
1.3621052631578947,0.3191489361702127,0.8975842246754837
1.3705263157894736,0.3191489361702127,0.8969902944318164
1.3789473684210527,0.3191489361702127,0.8963968268990357
1.3873684210526316,0.3191489361702127,0.8958038988366752
1.3957894736842105,0.3191489361702127,0.8952112784027122
1.4042105263157896,0.3191489361702127,0.8946192901539689
1.4126315789473685,0.3191489361702127,0.8940276354551315
1.4210526315789473,0.3191489361702127,0.8934364910237491
1.4294736842105262,0.3191489361702127,0.8928458224181668
1.4378947368421051,0.3191489361702127,0.8922556028119288
1.4463157894736842,0.3191489361702127,0.8916658591469968
1.454736842105263,0.3191489361702127,0.8910765349055509
1.4631578947368422,0.3191489361702127,0.8904877543445764
1.471578947368421,0.3191489361702127,0.889899379997587
1.48,0.3191489361702127,0.8893114200163836
1.4884210526315789,0.3191489361702127,0.8887239715149917
1.4968421052631578,0.3191489361702127,0.8881369316641212
1.5052631578947369,0.3191489361702127,0.887550344687952
1.5136842105263157,0.3191489361702127,0.8869643212246956
1.5221052631578948,0.3191489361702127,0.886378648497157
1.5305263157894737,0.3191489361702127,0.8857934431789545
1.5389473684210526,0.3191489361702127,0.885208726395831
1.5473684210526315,0.3191489361702127,0.8846244589085472
1.5557894736842104,0.3191489361702127,0.884040533535881
1.5642105263157895,0.3191489361702127,0.8834572160030802
1.5726315789473684,0.3191489361702127,0.882874270805587
1.5810526315789475,0.3191489361702127,0.8822917910147225
1.5894736842105264,0.3191489361702127,0.8817097525861755
1.5978947368421053,0.3191489361702127,0.9186549766745884
1.6063157894736841,0.3191489361702127,0.999476337260603
1.0,0.351063829787234,0.923612117767334
1.0084210526315789,0.351063829787234,0.9229991322954447
1.016842105263158,0.351063829787234,0.922386328268658
1.0252631578947369,0.351063829787234,0.9217740297617638
1.0336842105263158,0.351063829787234,0.9211621440581439
1.0421052631578946,0.351063829787234,0.9205508232344073
1.0505263157894738,0.351063829787234,0.9199397935644811
1.0589473684210526,0.351063829787234,0.9193294110091301
1.0673684210526315,0.351063829787234,0.9187194630485465
1.0757894736842104,0.351063829787234,0.918110025304486
1.0842105263157895,0.351063829787234,0.9175010304825264
1.0926315789473684,0.351063829787234,0.9168925434059929
1.1010526315789473,0.351063829787234,0.9162846888211789
1.1094736842105264,0.351063829787234,0.9156770589115695
1.1178947368421053,0.351063829787234,0.9150700579057229
1.1263157894736842,0.351063829787234,0.9144634653457615
1.134736842105263,0.351063829787234,0.9138573234067735
1.1431578947368422,0.351063829787234,0.9132517524240029
1.151578947368421,0.351063829787234,0.912646666173714
1.16,0.351063829787234,0.9120418941274693
1.168421052631579,0.351063829787234,0.911437511414988
1.176842105263158,0.351063829787234,0.910834118958519
1.1852631578947368,0.351063829787234,0.9102306058630347
1.1936842105263157,0.351063829787234,0.9096280700969146
1.2021052631578948,0.351063829787234,0.9090257988646044
1.2105263157894737,0.351063829787234,0.9084239855119449
1.2189473684210526,0.351063829787234,0.9078227074560345
1.2273684210526317,0.351063829787234,0.9072218557266751
1.2357894736842105,0.351063829787234,0.9066213350452017
1.2442105263157894,0.351063829787234,0.906021560706904
1.2526315789473683,0.351063829787234,0.9054222255954301
1.2610526315789474,0.351063829787234,0.9048231241658868
1.2694736842105263,0.351063829787234,0.9042246593016898
1.2778947368421052,0.351063829787234,0.9036266878547394
1.2863157894736843,0.351063829787234,0.9030291060516902
1.2947368421052632,0.351063829787234,0.902431968585006
1.303157894736842,0.351063829787234,0.9018354874870056
1.311578947368421,0.351063829787234,0.9012391417927574
1.32,0.351063829787234,0.9006437086954975
1.328421052631579,0.351063829787234,0.9000484982097987
1.3368421052631578,0.351063829787234,0.8994538079032282
1.345263157894737,0.351063829787234,0.8988595228383929
1.3536842105263158,0.351063829787234,0.8982656449079514
1.3621052631578947,0.351063829787234,0.8976723654195666
1.3705263157894736,0.351063829787234,0.8970795553650532
1.3789473684210527,0.351063829787234,0.8964871139851311
1.3873684210526316,0.351063829787234,0.8958953099217979
1.3957894736842105,0.351063829787234,0.895303813494138
1.4042105263157896,0.351063829787234,0.8947128696026994
1.4126315789473685,0.351063829787234,0.8941222964158442
1.4210526315789473,0.351063829787234,0.8935322565012029
1.4294736842105262,0.351063829787234,0.8929426903578133
1.4378947368421051,0.351063829787234,0.8923536114170929
1.4463157894736842,0.351063829787234,0.891764925328971
1.454736842105263,0.351063829787234,0.8911764621734619
1.4631578947368422,0.351063829787234,0.8905889853704139
1.471578947368421,0.351063829787234,0.890001777618636
1.48,0.351063829787234,0.8894148468934873
1.4884210526315789,0.351063829787234,0.8888286035062265
1.4968421052631578,0.351063829787234,0.8882426855770973
1.5052631578947369,0.351063829787234,0.8876573115467181
1.5136842105263157,0.351063829787234,0.8870723881527738
1.5221052631578948,0.351063829787234,0.8864878592048626
1.5305263157894737,0.351063829787234,0.8859038177288312
1.5389473684210526,0.351063829787234,0.8853202313139263
1.5473684210526315,0.351063829787234,0.8847370964904258
1.5557894736842104,0.351063829787234,0.8841544900224108
1.5642105263157895,0.351063829787234,0.8860865318838478
1.5726315789473684,0.351063829787234,0.9736385282594711
1.0,0.3829787234042553,0.9236608110022644
1.0084210526315789,0.3829787234042553,0.9230484376339518
1.016842105263158,0.3829787234042553,0.9224363864641418
1.0252631578947369,0.3829787234042553,0.9218247942244489
1.0336842105263158,0.3829787234042553,0.9212137255562993
1.0421052631578946,0.3829787234042553,0.9206032827542003
1.0505263157894738,0.3829787234042553,0.9199931201592335
1.0589473684210526,0.3829787234042553,0.9193834350444376
1.0673684210526315,0.3829787234042553,0.9187744097662289
1.0757894736842104,0.3829787234042553,0.9181657981207536
1.0842105263157895,0.3829787234042553,0.9175576525703946
1.0926315789473684,0.3829787234042553,0.9169501009200758
1.1010526315789473,0.3829787234042553,0.9163429284008089
1.1094736842105264,0.3829787234042553,0.9157363040894779
1.1178947368421053,0.3829787234042553,0.9151300915727916
1.1263157894736842,0.3829787234042553,0.9145244477085726
1.134736842105263,0.3829787234042553,0.913919208029256
1.1431578947368422,0.3829787234042553,0.9133144834677296
1.151578947368421,0.3829787234042553,0.9127102177571942
1.16,0.3829787234042553,0.9121065410809024
1.168421052631579,0.3829787234042553,0.9115032728404913
1.176842105263158,0.3829787234042553,0.9109001159667969
1.1852631578947368,0.3829787234042553,0.910298079252243
1.1936842105263157,0.3829787234042553,0.9096963582296667
1.2021052631578948,0.3829787234042553,0.9090950638792492
1.2105263157894737,0.3829787234042553,0.9084942052440965
1.2189473684210526,0.3829787234042553,0.9078937628701169
1.2273684210526317,0.3829787234042553,0.9072939166881042
1.2357894736842105,0.3829787234042553,0.9066944401693036
1.2442105263157894,0.3829787234042553,0.906095027923584
1.2526315789473683,0.3829787234042553,0.9054970742490696
1.2610526315789474,0.3829787234042553,0.9048990528535796
1.2694736842105263,0.3829787234042553,0.9043015013448894
1.2778947368421052,0.3829787234042553,0.9037044644355774
1.2863157894736843,0.3829787234042553,0.9031079849328307
1.2947368421052632,0.3829787234042553,0.902511897169461
1.303157894736842,0.3829787234042553,0.9019162913318723
1.311578947368421,0.3829787234042553,0.9013211836245318
1.32,0.3829787234042553,0.9007265851259945
1.328421052631579,0.3829787234042553,0.9001323506226981
1.3368421052631578,0.3829787234042553,0.8995386650194632
1.345263157894737,0.3829787234042553,0.8989454840175313
1.3536842105263158,0.3829787234042553,0.898352682350378
1.3621052631578947,0.3829787234042553,0.8977604860720021
1.3705263157894736,0.3829787234042553,0.897168660007992
1.3789473684210527,0.3829787234042553,0.8965772911615204
1.3873684210526316,0.3829787234042553,0.8959864303005816
1.3957894736842105,0.3829787234042553,0.895396110292495
1.4042105263157896,0.3829787234042553,0.8948061461560428
1.4126315789473685,0.3829787234042553,0.8942166566812375
1.4210526315789473,0.3829787234042553,0.893627823918905
1.4294736842105262,0.3829787234042553,0.8930393045238816
1.4378947368421051,0.3829787234042553,0.8924512674439029
1.4463157894736842,0.3829787234042553,0.8918637338101689
1.454736842105263,0.3829787234042553,0.8912766557759824
1.4631578947368422,0.3829787234042553,0.8906900660986139
1.471578947368421,0.3829787234042553,0.8901038504400276
1.48,0.3829787234042553,0.8895182649584967
1.4884210526315789,0.3829787234042553,0.8889329432859086
1.4968421052631578,0.3829787234042553,0.8883482347446261
1.5052631578947369,0.3829787234042553,0.8877640403861733
1.5136842105263157,0.3829787234042553,0.8871802177818608
1.5221052631578948,0.3829787234042553,0.8865968462150704
1.5305263157894737,0.3829787234042553,0.8860139854259614
1.5389473684210526,0.3829787234042553,0.9313808236411205
1.0,0.4148936170212766,0.9237092051016589
1.0084210526315789,0.4148936170212766,0.9230974315978528
1.016842105263158,0.4148936170212766,0.9224863648432802
1.0252631578947369,0.4148936170212766,0.9218755918573152
1.0336842105263158,0.4148936170212766,0.9212653683534882
1.0421052631578946,0.4148936170212766,0.9206555512273553
1.0505263157894738,0.4148936170212766,0.9200463704783033
1.0589473684210526,0.4148936170212766,0.9194376195091536
1.0673684210526315,0.4148936170212766,0.9188291728132754
1.0757894736842104,0.4148936170212766,0.9182216273666199
1.0842105263157895,0.4148936170212766,0.9176142138676369
1.0926315789473684,0.4148936170212766,0.9170075219408318
1.1010526315789473,0.4148936170212766,0.9164012675200865
1.1094736842105264,0.4148936170212766,0.915795415170578
1.1178947368421053,0.4148936170212766,0.9151900986862529
1.1263157894736842,0.4148936170212766,0.9145853690215517
1.134736842105263,0.4148936170212766,0.9139810837832556
1.1431578947368422,0.4148936170212766,0.9133771940196311
1.151578947368421,0.4148936170212766,0.9127738813576798
1.16,0.4148936170212766,0.9121711254201728
1.168421052631579,0.4148936170212766,0.9115686949817245
1.176842105263158,0.4148936170212766,0.9109667539560178
1.1852631578947368,0.4148936170212766,0.9103653691327054
1.1936842105263157,0.4148936170212766,0.9097644838275301
1.2021052631578948,0.4148936170212766,0.9091641043714844
1.2105263157894737,0.4148936170212766,0.9085641484125517
1.2189473684210526,0.4148936170212766,0.9079647666230812
1.2273684210526317,0.4148936170212766,0.9073657944109073
1.2357894736842105,0.4148936170212766,0.9067673290528546
1.2442105263157894,0.4148936170212766,0.9061693211206148
1.2526315789473683,0.4148936170212766,0.9055718140298268
1.2610526315789474,0.4148936170212766,0.9049748250117773
1.2694736842105263,0.4148936170212766,0.9043782911912785
1.2778947368421052,0.4148936170212766,0.903782244766262
1.2863157894736843,0.4148936170212766,0.9031867310568487
1.2947368421052632,0.4148936170212766,0.9025916814161974
1.303157894736842,0.4148936170212766,0.901996910572052
1.311578947368421,0.4148936170212766,0.9014029802101504
1.32,0.4148936170212766,0.9008092570584267
1.328421052631579,0.4148936170212766,0.9002162368278732
1.3368421052631578,0.4148936170212766,0.8996234938977068
1.345263157894737,0.4148936170212766,0.899031286961872
1.3536842105263158,0.4148936170212766,0.8984395188308554
1.3621052631578947,0.4148936170212766,0.8978483624832734
1.3705263157894736,0.4148936170212766,0.8972568511962891
1.3789473684210527,0.4148936170212766,0.8966670035515563
1.3873684210526316,0.4148936170212766,0.8960775062296307
1.3957894736842105,0.4148936170212766,0.8954882649886713
1.4042105263157896,0.4148936170212766,0.8948991294018924
1.4126315789473685,0.4148936170212766,0.8943109512329102
1.4210526315789473,0.4148936170212766,0.8937231411073299
1.4294736842105262,0.4148936170212766,0.893135666847229
1.4378947368421051,0.4148936170212766,0.892548782612721
1.4463157894736842,0.4148936170212766,0.8919624388227021
1.454736842105263,0.4148936170212766,0.8913764450708186
1.4631578947368422,0.4148936170212766,0.8907909422432567
1.471578947368421,0.4148936170212766,0.8902059346446549
1.48,0.4148936170212766,0.8896212958807155
1.4884210526315789,0.4148936170212766,0.8890372187152025
1.4968421052631578,0.4148936170212766,0.888453610785291
1.5052631578947369,0.4148936170212766,0.8878704140661284
1.5136842105263157,0.4148936170212766,0.9593460558971856
1.0,0.44680851063829785,0.9237575903543984
1.0084210526315789,0.44680851063829785,0.9231465660868707
1.016842105263158,0.44680851063829785,0.9225361527414861
1.0252631578947369,0.44680851063829785,0.9219262241822435
1.0336842105263158,0.44680851063829785,0.9213168919677628
1.0421052631578946,0.44680851063829785,0.9207076876409701
1.0505263157894738,0.44680851063829785,0.9200994641951183
1.0589473684210526,0.44680851063829785,0.9194914656636684
1.0673684210526315,0.44680851063829785,0.9188841213144769
1.0757894736842104,0.44680851063829785,0.9182771881451117
1.0842105263157895,0.44680851063829785,0.917670821977481
1.0926315789473684,0.44680851063829785,0.9170648723475097
1.1010526315789473,0.44680851063829785,0.916459381542154
1.1094736842105264,0.44680851063829785,0.9158545372574736
1.1178947368421053,0.44680851063829785,0.9152500549971592
1.1263157894736842,0.44680851063829785,0.91464616277608
1.134736842105263,0.44680851063829785,0.9140427504762556
1.1431578947368422,0.44680851063829785,0.9134398401092767
1.151578947368421,0.44680851063829785,0.912837338852114
1.16,0.44680851063829785,0.9122354316450583
1.168421052631579,0.44680851063829785,0.9116339703359699
1.176842105263158,0.44680851063829785,0.9110330346748015
1.1852631578947368,0.44680851063829785,0.9104324869031188
1.1936842105263157,0.44680851063829785,0.9098325147342621
1.2021052631578948,0.44680851063829785,0.9092331044494131
1.2105263157894737,0.44680851063829785,0.9086341041202104
1.2189473684210526,0.44680851063829785,0.9080356150661828
1.2273684210526317,0.44680851063829785,0.9074376042499352
1.2357894736842105,0.44680851063829785,0.9068400675841986
1.2442105263157894,0.44680851063829785,0.9062430233298073
1.2526315789473683,0.44680851063829785,0.9056466371121132
1.2610526315789474,0.44680851063829785,0.9050502775844507
1.2694736842105263,0.44680851063829785,0.9044550068510944
1.2778947368421052,0.44680851063829785,0.9038598238694249
1.2863157894736843,0.44680851063829785,0.9032652376336046
1.2947368421052632,0.44680851063829785,0.902671210448716
1.303157894736842,0.44680851063829785,0.9020774364471436
1.311578947368421,0.44680851063829785,0.9014845574865831
1.32,0.44680851063829785,0.9008918903182348
1.328421052631579,0.44680851063829785,0.9002995480550453
1.3368421052631578,0.44680851063829785,0.8997081303987216
1.345263157894737,0.44680851063829785,0.8991168736247346
1.3536842105263158,0.44680851063829785,0.8985262946025614
1.3621052631578947,0.44680851063829785,0.8979359860240947
1.3705263157894736,0.44680851063829785,0.8973463896909379
1.3789473684210527,0.44680851063829785,0.8967572748670136
1.3873684210526316,0.44680851063829785,0.8961684411242459
1.3957894736842105,0.44680851063829785,0.8955801971187611
1.4042105263157896,0.44680851063829785,0.8949924524358721
1.4126315789473685,0.44680851063829785,0.8944051349790243
1.4210526315789473,0.44680851063829785,0.8938183606305756
1.4294736842105262,0.44680851063829785,0.8932320178164446
1.4378947368421051,0.44680851063829785,0.8926461618193571
1.4463157894736842,0.44680851063829785,0.8920608091639224
1.454736842105263,0.44680851063829785,0.891475975994581
1.4631578947368422,0.44680851063829785,0.8908915632428034
1.471578947368421,0.44680851063829785,0.8903076395699827
1.48,0.44680851063829785,0.8897242214889047
1.4884210526315789,0.44680851063829785,0.9719534900559665
1.0,0.4787234042553191,0.9238057462471261
1.0084210526315789,0.4787234042553191,0.9231956068242653
1.016842105263158,0.4787234042553191,0.9225859873522495
1.0252631578947369,0.4787234042553191,0.9219768040347844
1.0336842105263158,0.4787234042553191,0.9213682114450421
1.0421052631578946,0.4787234042553191,0.9207598567008972
1.0505263157894738,0.4787234042553191,0.9201525224307261
1.0589473684210526,0.4787234042553191,0.9195454772589073
1.0673684210526315,0.4787234042553191,0.918938890168647
1.0757894736842104,0.4787234042553191,0.918332807976185
1.0842105263157895,0.4787234042553191,0.9177272026417995
1.0926315789473684,0.4787234042553191,0.9171220799807998
1.1010526315789473,0.4787234042553191,0.9165175557054681
1.1094736842105264,0.4787234042553191,0.9159135334202801
1.1178947368421053,0.4787234042553191,0.9153099330414989
1.1263157894736842,0.4787234042553191,0.9147068522106565
1.134736842105263,0.4787234042553191,0.9141043732252001
1.1431578947368422,0.4787234042553191,0.9135022161635789
1.151578947368421,0.4787234042553191,0.9129007568908492
1.16,0.4787234042553191,0.9122997341337395
1.168421052631579,0.4787234042553191,0.9116991760756719
1.176842105263158,0.4787234042553191,0.9110991066181668
1.1852631578947368,0.4787234042553191,0.910499576487382
1.1936842105263157,0.4787234042553191,0.9099004871432044
1.2021052631578948,0.4787234042553191,0.9093018751555064
1.2105263157894737,0.4787234042553191,0.908703869900819
1.2189473684210526,0.4787234042553191,0.9081063121275292
1.2273684210526317,0.4787234042553191,0.907509326935724
1.2357894736842105,0.4787234042553191,0.9069127477787333
1.2442105263157894,0.4787234042553191,0.9063162803649902
1.2526315789473683,0.4787234042553191,0.90572106421223
1.2610526315789474,0.4787234042553191,0.9051259879224745
1.2694736842105263,0.4787234042553191,0.9045313596707274
1.2778947368421052,0.4787234042553191,0.9039373604300636
1.2863157894736843,0.4787234042553191,0.9033437991174651
1.2947368421052632,0.4787234042553191,0.9027505963895237
1.303157894736842,0.4787234042553191,0.9021580820990494
1.311578947368421,0.4787234042553191,0.9015660360482798
1.32,0.4787234042553191,0.9009744078075528
1.328421052631579,0.4787234042553191,0.9003831893187453
1.3368421052631578,0.4787234042553191,0.8997925929543271
1.345263157894737,0.4787234042553191,0.8992023449391127
1.3536842105263158,0.4787234042553191,0.8986128596643539
1.3621052631578947,0.4787234042553191,0.8980235746021208
1.3705263157894736,0.4787234042553191,0.8974349974650977
1.3789473684210527,0.4787234042553191,0.89684692038918
1.3873684210526316,0.4787234042553191,0.8962592632033193
1.3957894736842105,0.4787234042553191,0.8956719457546569
1.4042105263157896,0.4787234042553191,0.8950852806146941
1.4126315789473685,0.4787234042553191,0.894499085854477
1.4210526315789473,0.4787234042553191,0.8939133199410207
1.4294736842105262,0.4787234042553191,0.893328033378566
1.4378947368421051,0.4787234042553191,0.8927433298786127
1.4463157894736842,0.4787234042553191,0.8921588659286499
1.454736842105263,0.4787234042553191,0.891575276851654
1.4631578947368422,0.4787234042553191,0.971143721973931
1.0,0.5106382978723404,0.92385383695364
1.0084210526315789,0.5106382978723404,0.9232446104952032
1.016842105263158,0.5106382978723404,0.9226357167635797
1.0252631578947369,0.5106382978723404,0.922027349457494
1.0336842105263158,0.5106382978723404,0.9214196411203375
1.0421052631578946,0.5106382978723404,0.9208122933387131
1.0505263157894738,0.5106382978723404,0.9202055161222233
1.0589473684210526,0.5106382978723404,0.9195993031626131
1.0673684210526315,0.5106382978723404,0.9189934580908812
1.0757894736842104,0.5106382978723404,0.9183882694123895
1.0842105263157895,0.5106382978723404,0.9177835513619357
1.0926315789473684,0.5106382978723404,0.9171793498107945
1.1010526315789473,0.5106382978723404,0.9165755966223514
1.1094736842105264,0.5106382978723404,0.9159722323529422
1.1178947368421053,0.5106382978723404,0.9153697144738544
1.1263157894736842,0.5106382978723404,0.9147672634571791
1.134736842105263,0.5106382978723404,0.9141657351210597
1.1431578947368422,0.5106382978723404,0.9135646889208147
1.151578947368421,0.5106382978723404,0.9129640056053177
1.16,0.5106382978723404,0.9123638982136981
1.168421052631579,0.5106382978723404,0.9117642659703051
1.176842105263158,0.5106382978723404,0.9111651080174852
1.1852631578947368,0.5106382978723404,0.9105664186317881
1.1936842105263157,0.5106382978723404,0.9099683015392657
1.2021052631578948,0.5106382978723404,0.9093704223623718
1.2105263157894737,0.5106382978723404,0.9087736022211175
1.2189473684210526,0.5106382978723404,0.9081768961586931
1.2273684210526317,0.5106382978723404,0.9075808525722096
1.2357894736842105,0.5106382978723404,0.9069852010852628
1.2442105263157894,0.5106382978723404,0.9063900996552547
1.2526315789473683,0.5106382978723404,0.9057955232792665
1.2610526315789474,0.5106382978723404,0.9052013130849446
1.2694736842105263,0.5106382978723404,0.9046077672383035
1.2778947368421052,0.5106382978723404,0.9040147099613023
1.2863157894736843,0.5106382978723404,0.903422053430404
1.2947368421052632,0.5106382978723404,0.902829967548314
1.303157894736842,0.5106382978723404,0.9022384881982362
1.311578947368421,0.5106382978723404,0.9016473318924909
1.32,0.5106382978723404,0.9010566007291345
1.328421052631579,0.5106382978723404,0.9004665089232731
1.3368421052631578,0.5106382978723404,0.8998769223680938
1.345263157894737,0.5106382978723404,0.8992878840699632
1.3536842105263158,0.5106382978723404,0.8986992548752823
1.3621052631578947,0.5106382978723404,0.8981110744553007
1.3705263157894736,0.5106382978723404,0.8975234659774287
1.3789473684210527,0.5106382978723404,0.896936356560218
1.3873684210526316,0.5106382978723404,0.8963497294662375
1.3957894736842105,0.5106382978723404,0.8957633972167969
1.4042105263157896,0.5106382978723404,0.895177924937343
1.4126315789473685,0.5106382978723404,0.8945928301773165
1.4210526315789473,0.5106382978723404,0.8940081436485343
1.4294736842105262,0.5106382978723404,0.8934239669306407
1.4378947368421051,0.5106382978723404,0.9585308365813034
1.0,0.5425531914893617,0.9239017963409424
1.0084210526315789,0.5425531914893617,0.9232934306746756
1.016842105263158,0.5425531914893617,0.9226853027939796
1.0252631578947369,0.5425531914893617,0.9220778852977674
1.0336842105263158,0.5425531914893617,0.9214708446488658
1.0421052631578946,0.5425531914893617,0.9208643470556126
1.0505263157894738,0.5425531914893617,0.920258313184604
1.0589473684210526,0.5425531914893617,0.9196529388427734
1.0673684210526315,0.5425531914893617,0.9190478324890137
1.0757894736842104,0.5425531914893617,0.918443678926451
1.0842105263157895,0.5425531914893617,0.9178397881969431
1.0926315789473684,0.5425531914893617,0.9172362978561068
1.1010526315789473,0.5425531914893617,0.9166335365298437
1.1094736842105264,0.5425531914893617,0.916031219211618
1.1178947368421053,0.5425531914893617,0.9154293758283529
1.1263157894736842,0.5425531914893617,0.9148280826657356
1.134736842105263,0.5425531914893617,0.9142272640192459
1.1431578947368422,0.5425531914893617,0.9136269092414295
1.151578947368421,0.5425531914893617,0.9130272199518004
1.16,0.5425531914893617,0.912427911272971
1.168421052631579,0.5425531914893617,0.9118292176235627
1.176842105263158,0.5425531914893617,0.9112309682923296
1.1852631578947368,0.5425531914893617,0.9106332451265189
1.1936842105263157,0.5425531914893617,0.9100360258444198
1.2021052631578948,0.5425531914893617,0.9094393537388896
1.2105263157894737,0.5425531914893617,0.9088431207783287
1.2189473684210526,0.5425531914893617,0.9082474720862592
1.2273684210526317,0.5425531914893617,0.9076522289251443
1.2357894736842105,0.5425531914893617,0.9070576095700744
1.2442105263157894,0.5425531914893617,0.9064634828146154
1.2526315789473683,0.5425531914893617,0.9058698508897578
1.2610526315789474,0.5425531914893617,0.90527665414902
1.2694736842105263,0.5425531914893617,0.9046839521906804
1.2778947368421052,0.5425531914893617,0.9040919197768744
1.2863157894736843,0.5425531914893617,0.9035001972224563
1.2947368421052632,0.5425531914893617,0.9029091638767568
1.303157894736842,0.5425531914893617,0.9023185978603578
1.311578947368421,0.5425531914893617,0.9017284598148763
1.32,0.5425531914893617,0.9011388720546165
1.328421052631579,0.5425531914893617,0.9005497352527527
1.3368421052631578,0.5425531914893617,0.8999611107028613
1.345263157894737,0.5425531914893617,0.8993730237853015
1.3536842105263158,0.5425531914893617,0.8987852928685243
1.3621052631578947,0.5425531914893617,0.8981983815056083
1.3705263157894736,0.5425531914893617,0.8976117588954367
1.3789473684210527,0.5425531914893617,0.8970255851718321
1.3873684210526316,0.5425531914893617,0.8964401520815954
1.3957894736842105,0.5425531914893617,0.8958550183997431
1.4042105263157896,0.5425531914893617,0.8952704216353595
1.4126315789473685,0.5425531914893617,0.9355357493595875
1.0,0.5744680851063829,0.9239499798422912
1.0084210526315789,0.5744680851063829,0.9233421872349936
1.016842105263158,0.5744680851063829,0.9227349821212556
1.0252631578947369,0.5744680851063829,0.9221282453627282
1.0336842105263158,0.5744680851063829,0.9215221415079213
1.0421052631578946,0.5744680851063829,0.9209163969881047
1.0505263157894738,0.5744680851063829,0.9203113020639648
1.0589473684210526,0.5744680851063829,0.919706608139677
1.0673684210526315,0.5744680851063829,0.9191025437739881
1.0757894736842104,0.5744680851063829,0.9184989855639287
1.0842105263157895,0.5744680851063829,0.9178956746472977
1.0926315789473684,0.5744680851063829,0.9172933692971128
1.1010526315789473,0.5744680851063829,0.9166912734217476
1.1094736842105264,0.5744680851063829,0.9160898843765608
1.1178947368421053,0.5744680851063829,0.9154888982857301
1.1263157894736842,0.5744680851063829,0.9148885215508926
1.134736842105263,0.5744680851063829,0.9142885133605887
1.1431578947368422,0.5744680851063829,0.913689206014169
1.151578947368421,0.5744680851063829,0.9130903408249651
1.16,0.5744680851063829,0.9124919175783361
1.168421052631579,0.5744680851063829,0.9118940736952936
1.176842105263158,0.5744680851063829,0.9112967632845539
1.1852631578947368,0.5744680851063829,0.9106997549533844
1.1936842105263157,0.5744680851063829,0.9101035594931091
1.2021052631578948,0.5744680851063829,0.909507848058638
1.2105263157894737,0.5744680851063829,0.9089126085118551
1.2189473684210526,0.5744680851063829,0.9083178869377662
1.2273684210526317,0.5744680851063829,0.9077236513121534
1.2357894736842105,0.5744680851063829,0.9071299050174275
1.2442105263157894,0.5744680851063829,0.9065365785500035
1.2526315789473683,0.5744680851063829,0.9059439810071126
1.2610526315789474,0.5744680851063829,0.905351819268617
1.2694736842105263,0.5744680851063829,0.9047601068741642
1.2778947368421052,0.5744680851063829,0.904168844222113
1.2863157894736843,0.5744680851063829,0.9035783859444564
1.2947368421052632,0.5744680851063829,0.9029881856313295
1.303157894736842,0.5744680851063829,0.9023985654303033
1.311578947368421,0.5744680851063829,0.9018092155456543
1.32,0.5744680851063829,0.9012208610056405
1.328421052631579,0.5744680851063829,0.9006328063896945
1.3368421052631578,0.5744680851063829,0.9000451852680271
1.345263157894737,0.5744680851063829,0.8994579315185547
1.3536842105263158,0.5744680851063829,0.8988715736495578
1.3621052631578947,0.5744680851063829,0.8982855082876995
1.3705263157894736,0.5744680851063829,0.897699773311615
1.3789473684210527,0.5744680851063829,0.8971148431155598
1.3873684210526316,0.5744680851063829,0.903459095400649
1.3957894736842105,0.5744680851063829,0.9824685288840556
1.0,0.6063829787234042,0.9239979347576082
1.0084210526315789,0.6063829787234042,0.9233909971972025
1.016842105263158,0.6063829787234042,0.9227845539599002
1.0252631578947369,0.6063829787234042,0.9221786148445972
1.0336842105263158,0.6063829787234042,0.9215731825352123
1.0421052631578946,0.6063829787234042,0.9209683559329278
1.0505263157894738,0.6063829787234042,0.9203640464811542
1.0589473684210526,0.6063829787234042,0.9197602872745847
1.0673684210526315,0.6063829787234042,0.9191569079976034
1.0757894736842104,0.6063829787234042,0.9185541741735506
1.0842105263157895,0.6063829787234042,0.9179518222799743
1.0926315789473684,0.6063829787234042,0.9173503508945942
1.1010526315789473,0.6063829787234042,0.9167491463867918
1.1094736842105264,0.6063829787234042,0.9161485732920482
1.1178947368421053,0.6063829787234042,0.9155483785943943
1.1263157894736842,0.6063829787234042,0.9149489086130416
1.134736842105263,0.6063829787234042,0.9143498219418689
1.1431578947368422,0.6063829787234042,0.9137513379109805
1.151578947368421,0.6063829787234042,0.9131532886785863
1.16,0.6063829787234042,0.9125557834777283
1.168421052631579,0.6063829787234042,0.9119588099310931
1.176842105263158,0.6063829787234042,0.9113624621013514
1.1852631578947368,0.6063829787234042,0.9107665498931965
1.1936842105263157,0.6063829787234042,0.910171178352357
1.2021052631578948,0.6063829787234042,0.9095762404613197
1.2105263157894737,0.6063829787234042,0.9089817926287651
1.2189473684210526,0.6063829787234042,0.9083881060942076
1.2273684210526317,0.6063829787234042,0.9077948369049409
1.2357894736842105,0.6063829787234042,0.9072019754821667
1.2442105263157894,0.6063829787234042,0.9066097852683015
1.2526315789473683,0.6063829787234042,0.9060180495198438
1.2610526315789474,0.6063829787234042,0.9054268368145131
1.2694736842105263,0.6063829787234042,0.904835939174518
1.2778947368421052,0.6063829787234042,0.9042458826907023
1.2863157894736843,0.6063829787234042,0.9036562647816027
1.2947368421052632,0.6063829787234042,0.9030671236305352
1.303157894736842,0.6063829787234042,0.9024784749690298
1.311578947368421,0.6063829787234042,0.9018904000504335
1.32,0.6063829787234042,0.9013027172759394
1.328421052631579,0.6063829787234042,0.9007156428633607
1.3368421052631578,0.6063829787234042,0.9001288414001465
1.345263157894737,0.6063829787234042,0.8995430767563448
1.3536842105263158,0.6063829787234042,0.8989574309498494
1.3621052631578947,0.6063829787234042,0.8983724578329202
1.3705263157894736,0.6063829787234042,0.9406091201799427
1.0,0.6382978723404255,0.9240458907643188
1.0084210526315789,0.6382978723404255,0.9234396913179808
1.016842105263158,0.6382978723404255,0.9228340499494152
1.0252631578947369,0.6382978723404255,0.9222289194131008
1.0336842105263158,0.6382978723404255,0.9216243648052114
1.0421052631578946,0.6382978723404255,0.9210202497115461
1.0505263157894738,0.6382978723404255,0.9204166457047904
1.0589473684210526,0.6382978723404255,0.9198135724291205
1.0673684210526315,0.6382978723404255,0.9192113042518031
1.0757894736842104,0.6382978723404255,0.9186094094884538
1.0842105263157895,0.6382978723404255,0.9180080448586523
1.0926315789473684,0.6382978723404255,0.9174072148844061
1.1010526315789473,0.6382978723404255,0.9168068820999906
1.1094736842105264,0.6382978723404255,0.916207066624338
1.1178947368421053,0.6382978723404255,0.9156078813857675
1.1263157894736842,0.6382978723404255,0.9150091622095715
1.134736842105263,0.6382978723404255,0.914410969263372
1.1431578947368422,0.6382978723404255,0.9138133603310052
1.151578947368421,0.6382978723404255,0.9132161363813793
1.16,0.6382978723404255,0.9126196515326228
1.168421052631579,0.6382978723404255,0.9120235815653359
1.176842105263158,0.6382978723404255,0.9114279148634523
1.1852631578947368,0.6382978723404255,0.9108329852406314
1.1936842105263157,0.6382978723404255,0.910238503907749
1.2021052631578948,0.6382978723404255,0.9096445860059248
1.2105263157894737,0.6382978723404255,0.9090512096890961
1.2189473684210526,0.6382978723404255,0.9084582867644713
1.2273684210526317,0.6382978723404255,0.9078659119231816
1.2357894736842105,0.6382978723404255,0.9072740077936032
1.2442105263157894,0.6382978723404255,0.9066827754732003
1.2526315789473683,0.6382978723404255,0.9060919925987037
1.2610526315789474,0.6382978723404255,0.9055017170176143
1.2694736842105263,0.6382978723404255,0.9049119916926429
1.2778947368421052,0.6382978723404255,0.9043226834619418
1.2863157894736843,0.6382978723404255,0.9037340131471865
1.2947368421052632,0.6382978723404255,0.9031459246352824
1.303157894736842,0.6382978723404255,0.9025582125259461
1.311578947368421,0.6382978723404255,0.9019709226704435
1.32,0.6382978723404255,0.901384503117697
1.328421052631579,0.6382978723404255,0.9007983680803591
1.3368421052631578,0.6382978723404255,0.9002128839501893
1.345263157894737,0.6382978723404255,0.8996278047779924
1.3536842105263158,0.6382978723404255,0.9693838367829812
1.0,0.6702127659574467,0.924093726584033
1.0084210526315789,0.6702127659574467,0.923488378991351
1.016842105263158,0.6702127659574467,0.9228834810646731
1.0252631578947369,0.6702127659574467,0.9222791230013172
1.0336842105263158,0.6702127659574467,0.9216753432147016
1.0421052631578946,0.6702127659574467,0.9210721264835229
1.0505263157894738,0.6702127659574467,0.920469282194972
1.0589473684210526,0.6702127659574467,0.919867204052025
1.0673684210526315,0.6702127659574467,0.9192655291353731
1.0757894736842104,0.6702127659574467,0.9186644390938454
1.0842105263157895,0.6702127659574467,0.9180640094155024
1.0926315789473684,0.6702127659574467,0.9174640178980553
1.1010526315789473,0.6702127659574467,0.9168644901119478
1.1094736842105264,0.6702127659574467,0.9162655323261788
1.1178947368421053,0.6702127659574467,0.9156671775699579
1.1263157894736842,0.6702127659574467,0.9150693584533656
1.134736842105263,0.6702127659574467,0.9144719528676433
1.1431578947368422,0.6702127659574467,0.9138750873935351
1.151578947368421,0.6702127659574467,0.9132790037356244
1.16,0.6702127659574467,0.9126832476376876
1.168421052631579,0.6702127659574467,0.9120881594917591
1.176842105263158,0.6702127659574467,0.9114935615225477
1.1852631578947368,0.6702127659574467,0.9108993896234097
1.1936842105263157,0.6702127659574467,0.9103055000159657
1.2021052631578948,0.6702127659574467,0.9097127349159564
1.2105263157894737,0.6702127659574467,0.9091202000054182
1.2189473684210526,0.6702127659574467,0.908528369056512
1.2273684210526317,0.6702127659574467,0.9079367788490345
1.2357894736842105,0.6702127659574467,0.907346027431231
1.2442105263157894,0.6702127659574467,0.9067556099817011
1.2526315789473683,0.6702127659574467,0.9061658238470045
1.2610526315789474,0.6702127659574467,0.9055764526128769
1.2694736842105263,0.6702127659574467,0.904987722912665
1.2778947368421052,0.6702127659574467,0.9043993949890137
1.2863157894736843,0.6702127659574467,0.9038116930278193
1.2947368421052632,0.6702127659574467,0.9032244300396997
1.303157894736842,0.6702127659574467,0.9026378408379969
1.311578947368421,0.6702127659574467,0.9020517542967355
1.32,0.6702127659574467,0.901466086686014
1.328421052631579,0.6702127659574467,0.9124454250559211
1.3368421052631578,0.6702127659574467,0.9903469504051827
1.0,0.702127659574468,0.924141495674121
1.0084210526315789,0.702127659574468,0.9235369416428512
1.016842105263158,0.702127659574468,0.9229328295632513
1.0252631578947369,0.702127659574468,0.922329155713669
1.0336842105263158,0.702127659574468,0.9217262946203846
1.0421052631578946,0.702127659574468,0.921123800038913
1.0505263157894738,0.702127659574468,0.920521974593612
1.0589473684210526,0.702127659574468,0.9199205031036399
1.0673684210526315,0.702127659574468,0.9193197916765712
1.0757894736842104,0.702127659574468,0.9187195203094234
1.0842105263157895,0.702127659574468,0.9181198122769274
1.0926315789473684,0.702127659574468,0.9175205778865347
1.1010526315789473,0.702127659574468,0.9169219396590051
1.1094736842105264,0.702127659574468,0.9163240213028985
1.1178947368421053,0.702127659574468,0.9157263538509142
1.1263157894736842,0.702127659574468,0.9151294082594177
1.134736842105263,0.702127659574468,0.9145328399599748
1.1431578947368422,0.702127659574468,0.9139370465290995
1.151578947368421,0.702127659574468,0.9133416324448262
1.16,0.702127659574468,0.9127467758062267
1.168421052631579,0.702127659574468,0.9121524539659731
1.176842105263158,0.702127659574468,0.9115588993399797
1.1852631578947368,0.702127659574468,0.9109656734590317
1.1936842105263157,0.702127659574468,0.910372969187847
1.2021052631578948,0.702127659574468,0.9097809034064994
1.2105263157894737,0.702127659574468,0.9091893435806924
1.2189473684210526,0.702127659574468,0.9085983354625569
1.2273684210526317,0.702127659574468,0.9080077954486114
1.2357894736842105,0.702127659574468,0.9074177590655381
1.2442105263157894,0.702127659574468,0.90682836783526
1.2526315789473683,0.702127659574468,0.906239530109815
1.2610526315789474,0.702127659574468,0.9056511524877351
1.2694736842105263,0.702127659574468,0.9050632118014619
1.2778947368421052,0.702127659574468,0.9044760344850147
1.2863157894736843,0.702127659574468,0.9038892612088603
1.2947368421052632,0.702127659574468,0.9033030199116183
1.303157894736842,0.702127659574468,0.902717370569917
1.311578947368421,0.702127659574468,0.9259064863172171
1.0,0.7340425531914893,0.9241892808940975
1.0084210526315789,0.7340425531914893,0.923585424261546
1.016842105263158,0.7340425531914893,0.9229821180952058
1.0252631578947369,0.7340425531914893,0.9223793759174441
1.0336842105263158,0.7340425531914893,0.921777132920397
1.0421052631578946,0.7340425531914893,0.9211755397282104
1.0505263157894738,0.7340425531914893,0.9205742701597046
1.0589473684210526,0.7340425531914893,0.9199738810602867
1.0673684210526315,0.7340425531914893,0.9193737864488867
1.0757894736842104,0.7340425531914893,0.9187743647671596
1.0842105263157895,0.7340425531914893,0.9181755781810352
1.0926315789473684,0.7340425531914893,0.9175772983880961
1.1010526315789473,0.7340425531914893,0.9169794572981118
1.1094736842105264,0.7340425531914893,0.9163822626032925
1.1178947368421053,0.7340425531914893,0.9157852800562978
1.1263157894736842,0.7340425531914893,0.9151892363879597
1.134736842105263,0.7340425531914893,0.9145937839130056
1.1431578947368422,0.7340425531914893,0.913998780511065
1.151578947368421,0.7340425531914893,0.9134043238318554
1.16,0.7340425531914893,0.9128103190996626
1.168421052631579,0.7340425531914893,0.9122169622241927
1.176842105263158,0.7340425531914893,0.9116241678584629
1.1852631578947368,0.7340425531914893,0.9110318664170336
1.1936842105263157,0.7340425531914893,0.9104401473350663
1.2021052631578948,0.7340425531914893,0.9098489235293528
1.2105263157894737,0.7340425531914893,0.909258278094967
1.2189473684210526,0.7340425531914893,0.908668056008537
1.2273684210526317,0.7340425531914893,0.9080786108988832
1.2357894736842105,0.7340425531914893,0.907489496573362
1.2442105263157894,0.7340425531914893,0.9069010110260933
1.2526315789473683,0.7340425531914893,0.906313001873059
1.2610526315789474,0.7340425531914893,0.9057257175454652
1.2694736842105263,0.7340425531914893,0.9051387859990427
1.2778947368421052,0.7340425531914893,0.9045524485418355
1.2863157894736843,0.7340425531914893,0.903966647812922
1.2947368421052632,0.7340425531914893,0.9326807004426882
1.0,0.7659574468085106,0.9242368602763236
1.0084210526315789,0.7659574468085106,0.9236337952097529
1.016842105263158,0.7659574468085106,0.9230313385251065
1.0252631578947369,0.7659574468085106,0.9224293143088289
1.0336842105263158,0.7659574468085106,0.9218279831120526
1.0421052631578946,0.7659574468085106,0.921226929025579
1.0505263157894738,0.7659574468085106,0.9206266249502733
1.0589473684210526,0.7659574468085106,0.9200268950344253
1.0673684210526315,0.7659574468085106,0.9194279909143006
1.0757894736842104,0.7659574468085106,0.918829305142026
1.0842105263157895,0.7659574468085106,0.9182312498205647
1.0926315789473684,0.7659574468085106,0.9176335334777832
1.1010526315789473,0.7659574468085106,0.9170367734022875
1.1094736842105264,0.7659574468085106,0.9164405167111909
1.1178947368421053,0.7659574468085106,0.9158444829035943
1.1263157894736842,0.7659574468085106,0.9152491092099808
1.134736842105263,0.7659574468085106,0.9146546523634242
1.1431578947368422,0.7659574468085106,0.9140604062031343
1.151578947368421,0.7659574468085106,0.9134669010700236
1.16,0.7659574468085106,0.9128738068184248
1.168421052631579,0.7659574468085106,0.9122812123896438
1.176842105263158,0.7659574468085106,0.9116892734891735
1.1852631578947368,0.7659574468085106,0.9110980034229215
1.1936842105263157,0.7659574468085106,0.9105070137156872
1.2021052631578948,0.7659574468085106,0.9099163999744633
1.2105263157894737,0.7659574468085106,0.9093270137973377
1.2189473684210526,0.7659574468085106,0.9087376556635718
1.2273684210526317,0.7659574468085106,0.9081487581133842
1.2357894736842105,0.7659574468085106,0.9075611164453221
1.2442105263157894,0.7659574468085106,0.9069735715374918
1.2526315789473683,0.7659574468085106,0.9063865580837955
1.2610526315789474,0.7659574468085106,0.9057998654307085
1.2694736842105263,0.7659574468085106,0.9052141462534564
1.2778947368421052,0.7659574468085106,0.9332149163774375
1.0,0.7978723404255319,0.9242845239532471
1.0084210526315789,0.7978723404255319,0.9236821222657454
1.016842105263158,0.7978723404255319,0.9230805039414918
1.0252631578947369,0.7978723404255319,0.9224792942532076
1.0336842105263158,0.7978723404255319,0.9218783378601074
1.0421052631578946,0.7978723404255319,0.9212785892941611
1.0505263157894738,0.7978723404255319,0.9206791447604701
1.0589473684210526,0.7978723404255319,0.9200802497680343
1.0673684210526315,0.7978723404255319,0.9194817728111957
1.0757894736842104,0.7978723404255319,0.9188839940443359
1.0842105263157895,0.7978723404255319,0.9182869270489391
1.0926315789473684,0.7978723404255319,0.9176902483495724
1.1010526315789473,0.7978723404255319,0.9170941719839902
1.1094736842105264,0.7978723404255319,0.9164985095085285
1.1178947368421053,0.7978723404255319,0.9159034702306599
1.1263157894736842,0.7978723404255319,0.9153092226197259
1.134736842105263,0.7978723404255319,0.9147152963350891
1.1431578947368422,0.7978723404255319,0.9141219181765337
1.151578947368421,0.7978723404255319,0.9135291423881426
1.16,0.7978723404255319,0.9129371643075501
1.168421052631579,0.7978723404255319,0.9123455304716117
1.176842105263158,0.7978723404255319,0.9117543682041287
1.1852631578947368,0.7978723404255319,0.9111640453347718
1.1936842105263157,0.7978723404255319,0.9105739853730483
1.2021052631578948,0.7978723404255319,0.9099845891441873
1.2105263157894737,0.7978723404255319,0.9093957645827686
1.2189473684210526,0.7978723404255319,0.9088074185983714
1.2273684210526317,0.7978723404255319,0.9082197085399457
1.2357894736842105,0.7978723404255319,0.9076324701309204
1.2442105263157894,0.7978723404255319,0.9070458937248986
1.2526315789473683,0.7978723404255319,0.9064598169061355
1.2610526315789474,0.7978723404255319,0.9279391574364126
1.0,0.8297872340425532,0.924331957196955
1.0084210526315789,0.8297872340425532,0.9237305317155915
1.016842105263158,0.8297872340425532,0.9231294207202154
1.0252631578947369,0.8297872340425532,0.9225289523019455
1.0336842105263158,0.8297872340425532,0.9219291805775356
1.0421052631578946,0.8297872340425532,0.9213299699904383
1.0505263157894738,0.8297872340425532,0.9207314489785858
1.0589473684210526,0.8297872340425532,0.9201332979755534
1.0673684210526315,0.8297872340425532,0.919535681776324
1.0757894736842104,0.8297872340425532,0.918938878924564
1.0842105263157895,0.8297872340425532,0.918342393392777
1.0926315789473684,0.8297872340425532,0.9177465933289568
1.1010526315789473,0.8297872340425532,0.9171512645443727
1.1094736842105264,0.8297872340425532,0.9165566039409896
1.1178947368421053,0.8297872340425532,0.9159624227022505
1.1263157894736842,0.8297872340425532,0.9153689742770439
1.134736842105263,0.8297872340425532,0.9147759054176277
1.1431578947368422,0.8297872340425532,0.9141835572700074
1.151578947368421,0.8297872340425532,0.9135916503837507
1.16,0.8297872340425532,0.9130003564196159
1.168421052631579,0.8297872340425532,0.9124096224632012
1.176842105263158,0.8297872340425532,0.9118194383054288
1.1852631578947368,0.8297872340425532,0.9112297882920757
1.1936842105263157,0.8297872340425532,0.9106408134402955
1.2021052631578948,0.8297872340425532,0.9100522851813366
1.2105263157894737,0.8297872340425532,0.9094642986310646
1.2189473684210526,0.8297872340425532,0.9088769462432538
1.2273684210526317,0.8297872340425532,0.9082901478086569
1.2357894736842105,0.8297872340425532,0.9077036362141371
1.2442105263157894,0.8297872340425532,0.9172726571559906
1.2526315789473683,0.8297872340425532,0.994495186828317
1.0,0.8617021276595744,0.9243795236270671
1.0084210526315789,0.8617021276595744,0.9237788021755478
1.016842105263158,0.8617021276595744,0.9231784920557402
1.0252631578947369,0.8617021276595744,0.9225789823185551
1.0336842105263158,0.8617021276595744,0.9219799681168297
1.0421052631578946,0.8617021276595744,0.9213815350967707
1.0505263157894738,0.8617021276595744,0.9207835280103609
1.0589473684210526,0.8617021276595744,0.9201862642912602
1.0673684210526315,0.8617021276595744,0.9195895137891057
1.0757894736842104,0.8617021276595744,0.9189933072775602
1.0842105263157895,0.8617021276595744,0.9183977236352803
1.0926315789473684,0.8617021276595744,0.9178026167792268
1.1010526315789473,0.8617021276595744,0.9172084107403862
1.1094736842105264,0.8617021276595744,0.916614610603574
1.1178947368421053,0.8617021276595744,0.9160212966089603
1.1263157894736842,0.8617021276595744,0.9154286396378666
1.134736842105263,0.8617021276595744,0.9148364872680759
1.1431578947368422,0.8617021276595744,0.9142449246155593
1.151578947368421,0.8617021276595744,0.9136539045402969
1.16,0.8617021276595744,0.9130634816310703
1.168421052631579,0.8617021276595744,0.9124735658933787
1.176842105263158,0.8617021276595744,0.91188431946739
1.1852631578947368,0.8617021276595744,0.9112955746095395
1.1936842105263157,0.8617021276595744,0.9107074169805855
1.2021052631578948,0.8617021276595744,0.910119652740832
1.2105263157894737,0.8617021276595744,0.9095327258037287
1.2189473684210526,0.8617021276595744,0.9089462757110596
1.2273684210526317,0.8617021276595744,0.9083602125683683
1.2357894736842105,0.8617021276595744,0.9782071805584565
1.0,0.8936170212765957,0.9244269083746985
1.0084210526315789,0.8936170212765957,0.9238269328652677
1.016842105263158,0.8936170212765957,0.9232275530448533
1.0252631578947369,0.8936170212765957,0.9226287108085671
1.0336842105263158,0.8936170212765957,0.9220304786704219
1.0421052631578946,0.8936170212765957,0.9214326873388927
1.0505263157894738,0.8936170212765957,0.9208357637999143
1.0589473684210526,0.8936170212765957,0.9202389859556206
1.0673684210526315,0.8936170212765957,0.9196432924300098
1.0757894736842104,0.8936170212765957,0.9190479353837873
1.0842105263157895,0.8936170212765957,0.9184532097833653
1.0926315789473684,0.8936170212765957,0.9178590765604895
1.1010526315789473,0.8936170212765957,0.9172652865527198
1.1094736842105264,0.8936170212765957,0.916672451156046
1.1178947368421053,0.8936170212765957,0.9160799905648673
1.1263157894736842,0.8936170212765957,0.9154882151642596
1.134736842105263,0.8936170212765957,0.9148968740310011
1.1431578947368422,0.8936170212765957,0.9143061669983581
1.151578947368421,0.8936170212765957,0.9137160964337454
1.16,0.8936170212765957,0.9131259917048737
1.168421052631579,0.8936170212765957,0.9125375352168703
1.176842105263158,0.8936170212765957,0.9119486138224602
1.1852631578947368,0.8936170212765957,0.9113606475293636
1.1936842105263157,0.8936170212765957,0.9107739795244925
1.2021052631578948,0.8936170212765957,0.9101873046647597
1.2105263157894737,0.8936170212765957,0.9096006080508232
1.2189473684210526,0.8936170212765957,0.9571791068019593
1.0,0.925531914893617,0.9244742392911576
1.0084210526315789,0.925531914893617,0.9238750729309686
1.016842105263158,0.925531914893617,0.9232762910605743
1.0252631578947369,0.925531914893617,0.9226781561992539
1.0336842105263158,0.925531914893617,0.9220809638945866
1.0421052631578946,0.925531914893617,0.9214840607082806
1.0505263157894738,0.925531914893617,0.9208877232640589
1.0589473684210526,0.925531914893617,0.9202918987575686
1.0673684210526315,0.925531914893617,0.9196969110971622
1.0757894736842104,0.925531914893617,0.9191023108433001
1.0842105263157895,0.925531914893617,0.9185085277767939
1.0926315789473684,0.925531914893617,0.9179151837561221
1.1010526315789473,0.925531914893617,0.917322435963797
1.1094736842105264,0.925531914893617,0.9167299045875552
1.1178947368421053,0.925531914893617,0.916138172004139
1.1263157894736842,0.925531914893617,0.9155476895984975
1.134736842105263,0.925531914893617,0.9149572426713348
1.1431578947368422,0.925531914893617,0.9143673856879104
1.151578947368421,0.925531914893617,0.9137781579092916
1.16,0.925531914893617,0.9131892286077345
1.168421052631579,0.925531914893617,0.9126012705937683
1.176842105263158,0.925531914893617,0.9120138010639494
1.1852631578947368,0.925531914893617,0.9114267818640656
1.1936842105263157,0.925531914893617,0.910840467116941
1.2021052631578948,0.925531914893617,0.9318179567726474
1.0,0.9574468085106382,0.9245211477318662
1.0084210526315789,0.9574468085106382,0.9239229559898376
1.016842105263158,0.9574468085106382,0.9233253004504149
1.0252631578947369,0.9574468085106382,0.9227279550250387
1.0336842105263158,0.9574468085106382,0.9221313397292761
1.0421052631578946,0.9574468085106382,0.9215352087030624
1.0505263157894738,0.9574468085106382,0.9209397043887293
1.0589473684210526,0.9574468085106382,0.9203448511752867
1.0673684210526315,0.9574468085106382,0.9197505787096816
1.0757894736842104,0.9574468085106382,0.9191563129425049
1.0842105263157895,0.9574468085106382,0.9185637971759206
1.0926315789473684,0.9574468085106382,0.9179712721625037
1.1010526315789473,0.9574468085106382,0.9173792530782521
1.1094736842105264,0.9574468085106382,0.916787862763158
1.1178947368421053,0.9574468085106382,0.9161973157906687
1.1263157894736842,0.9574468085106382,0.9156070427970917
1.134736842105263,0.9574468085106382,0.915017471776082
1.1431578947368422,0.9574468085106382,0.9144285321253847
1.151578947368421,0.9574468085106382,0.913840023742523
1.16,0.9574468085106382,0.9132519345712353
1.168421052631579,0.9574468085106382,0.9126650160496865
1.176842105263158,0.9574468085106382,0.9120783152220611
1.1852631578947368,0.9574468085106382,0.9114922955786824
1.1936842105263157,0.9574468085106382,0.9792409837618834
1.0,0.9893617021276595,0.924568810771234
1.0084210526315789,0.9893617021276595,0.9239711761483704
1.016842105263158,0.9893617021276595,0.923373907480709
1.0252631578947369,0.9893617021276595,0.9227775944173118
1.0336842105263158,0.9893617021276595,0.9221816061090067
1.0421052631578946,0.9893617021276595,0.9215861968614263
1.0505263157894738,0.9893617021276595,0.9209916602421799
1.0589473684210526,0.9893617021276595,0.9203975762766277
1.0673684210526315,0.9893617021276595,0.9198041562949584
1.0757894736842104,0.9893617021276595,0.9192109070645529
1.0842105263157895,0.9893617021276595,0.9186188556413981
1.0926315789473684,0.9893617021276595,0.9180268049076403
1.1010526315789473,0.9893617021276595,0.9174360743481884
1.1094736842105264,0.9893617021276595,0.9168455615781568
1.1178947368421053,0.9893617021276595,0.9162556525516266
1.1263157894736842,0.9893617021276595,0.9156661758861446
1.134736842105263,0.9893617021276595,0.9150776189844692
1.1431578947368422,0.9893617021276595,0.9144887924012437
1.151578947368421,0.9893617021276595,0.9139018641999428
1.16,0.9893617021276595,0.9133149383123964
1.168421052631579,0.9893617021276595,0.9127286672601258
1.176842105263158,0.9893617021276595,0.9451426111454566
1.0,1.0212765957446808,0.9246158709456722
1.0084210526315789,1.0212765957446808,0.9240189487900352
1.016842105263158,1.0212765957446808,0.9234227131819353
1.0252631578947369,1.0212765957446808,0.9228269846771582
1.0336842105263158,1.0212765957446808,0.9222316592931747
1.0421052631578946,1.0212765957446808,0.9216374312827611
1.0505263157894738,1.0212765957446808,0.9210435161621717
1.0589473684210526,1.0212765957446808,0.9204502242710078
1.0673684210526315,1.0212765957446808,0.9198575482123488
1.0757894736842104,1.0212765957446808,0.9192654707358088
1.0842105263157895,1.0212765957446808,0.9186739699780446
1.0926315789473684,1.0212765957446808,0.918082706626592
1.1010526315789473,1.0212765957446808,0.9174927744879824
1.1094736842105264,1.0212765957446808,0.916903018951416
1.1178947368421053,1.0212765957446808,0.9163140348946399
1.1263157894736842,1.0212765957446808,0.9157254090496281
1.134736842105263,1.0212765957446808,0.9151376738445833
1.1431578947368422,1.0212765957446808,0.9145504834750682
1.151578947368421,1.0212765957446808,0.913963703202171
1.16,1.0212765957446808,0.9133776724420386
1.168421052631579,1.0212765957446808,0.9848901233162906
1.0,1.053191489361702,0.9246630676798304
1.0084210526315789,1.053191489361702,0.9240668208694842
1.016842105263158,1.053191489361702,0.9234712334937285
1.0252631578947369,1.053191489361702,0.9228763907867688
1.0336842105263158,1.053191489361702,0.9222820838840562
1.0421052631578946,1.053191489361702,0.9216882549226284
1.0505263157894738,1.053191489361702,0.9210952109988284
1.0589473684210526,1.053191489361702,0.9205027832031192
1.0673684210526315,1.053191489361702,0.9199108106531639
1.0757894736842104,1.053191489361702,0.9193196259702745
1.0842105263157895,1.053191489361702,0.9187289463816342
1.0926315789473684,1.053191489361702,0.9181388019351289
1.1010526315789473,1.053191489361702,0.9175493845214078
1.1094736842105264,1.053191489361702,0.9169606046079934
1.1178947368421053,1.053191489361702,0.9163721794238882
1.1263157894736842,1.053191489361702,0.9157847648029929
1.134736842105263,1.053191489361702,0.9151976816829119
1.1431578947368422,1.053191489361702,0.9146108605855261
1.151578947368421,1.053191489361702,0.9430430263028029
1.0,1.0851063829787233,0.9247097967745503
1.0084210526315789,1.0851063829787233,0.9241147168222597
1.016842105263158,1.0851063829787233,0.9235199294089398
1.0252631578947369,1.0851063829787233,0.9229257678871363
1.0336842105263158,1.0851063829787233,0.9223322160250973
1.0421052631578946,1.0851063829787233,0.9217391759102611
1.0505263157894738,1.0851063829787233,0.9211470047312105
1.0589473684210526,1.0851063829787233,0.9205552329540296
1.0673684210526315,1.0851063829787233,0.9199641327941208
1.0757894736842104,1.0851063829787233,0.9193736910447114
1.0842105263157895,1.0851063829787233,0.9187838629904945
1.0926315789473684,1.0851063829787233,0.9181946138123749
1.1010526315789473,1.0851063829787233,0.9176059600094959
1.1094736842105264,1.0851063829787233,0.9170178171461885
1.1178947368421053,1.0851063829787233,0.916430544085415
1.1263157894736842,1.0851063829787233,0.9158430098905228
1.134736842105263,1.0851063829787233,0.9152575461384913
1.1431578947368422,1.0851063829787233,0.9755810047199702
1.0,1.1170212765957446,0.9247570363804698
1.0084210526315789,1.1170212765957446,0.9241623867237649
1.016842105263158,1.1170212765957446,0.9235684087216214
1.0252631578947369,1.1170212765957446,0.9229750451095242
1.0336842105263158,1.1170212765957446,0.9223823547445136
1.0421052631578946,1.1170212765957446,0.9217901252141019
1.0505263157894738,1.1170212765957446,0.9211986191603501
1.0589473684210526,1.1170212765957446,0.9206076949658382
1.0673684210526315,1.1170212765957446,0.9200173967929004
1.0757894736842104,1.1170212765957446,0.9194276253547287
1.0842105263157895,1.1170212765957446,0.9188386905998414
1.0926315789473684,1.1170212765957446,0.9182491302490234
1.1010526315789473,1.1170212765957446,0.9176624604060635
1.1094736842105264,1.1170212765957446,0.9170753071093714
1.1178947368421053,1.1170212765957446,0.9164886712151201
1.1263157894736842,1.1170212765957446,0.9269910084576622
1.0,1.1489361702127658,0.9248039722406247
1.0084210526315789,1.1489361702127658,0.9242101532336164
1.016842105263158,1.1489361702127658,0.9236168880997866
1.0252631578947369,1.1489361702127658,0.9230242904768602
1.0336842105263158,1.1489361702127658,0.9224322102945735
1.0421052631578946,1.1489361702127658,0.9218409061613784
1.0505263157894738,1.1489361702127658,0.9212501680140122
1.0589473684210526,1.1489361702127658,0.9206598326491076
1.0673684210526315,1.1489361702127658,0.9200704096656409
1.0757894736842104,1.1489361702127658,0.9194814076945477
1.0842105263157895,1.1489361702127658,0.9188934603544112
1.0926315789473684,1.1489361702127658,0.9183055602979948
1.1010526315789473,1.1489361702127658,0.9177188580533766
1.1094736842105264,1.1489361702127658,0.9171323748014402
1.1178947368421053,1.1489361702127658,0.9528088318029404
1.0,1.180851063829787,0.9248504638089798
1.0084210526315789,1.180851063829787,0.9242572784423828
1.016842105263158,1.180851063829787,0.9236652242689161
1.0252631578947369,1.180851063829787,0.9230734408065473
1.0336842105263158,1.180851063829787,0.9224822067199057
1.0421052631578946,1.180851063829787,0.9218916203835761
1.0505263157894738,1.180851063829787,0.9213017001920889
1.0589473684210526,1.180851063829787,0.920712313567492
1.0673684210526315,1.180851063829787,0.9201232008335865
1.0757894736842104,1.180851063829787,0.9195353834620619
1.0842105263157895,1.180851063829787,0.918948139317763
1.0926315789473684,1.180851063829787,0.9183612465558326
1.1010526315789473,1.180851063829787,0.917774555971846
1.1094736842105264,1.180851063829787,0.9760471622148543
1.0,1.2127659574468084,0.9248977380730139
1.0084210526315789,1.2127659574468084,0.9243053868422066
1.016842105263158,1.2127659574468084,0.9237135717394267
1.0252631578947369,1.2127659574468084,0.9231225848207032
1.0336842105263158,1.2127659574468084,0.9225320164032382
1.0421052631578946,1.2127659574468084,0.9219421855787004
1.0505263157894738,1.2127659574468084,0.9213528630016299
1.0589473684210526,1.2127659574468084,0.9207641736111327
1.0673684210526315,1.2127659574468084,0.9201766116784711
1.0757894736842104,1.2127659574468084,0.9195889820111915
1.0842105263157895,1.2127659574468084,0.9190027261729483
1.0926315789473684,1.2127659574468084,0.9184167224475459
1.1010526315789473,1.2127659574468084,0.9967372872870328
1.0,1.2446808510638296,0.924944475294069
1.0084210526315789,1.2446808510638296,0.924352827128132
1.016842105263158,1.2446808510638296,0.923761843569082
1.0252631578947369,1.2446808510638296,0.9231715152109246
1.0336842105263158,1.2446808510638296,0.9225818321119732
1.0421052631578946,1.2446808510638296,0.9219927883123091
1.0505263157894738,1.2446808510638296,0.9214038513600826
1.0589473684210526,1.2446808510638296,0.920816670172826
1.0673684210526315,1.2446808510638296,0.9202289282984566
1.0757894736842104,1.2446808510638296,0.9196430733891248
1.0842105263157895,1.2446808510638296,0.9353000609116862
1.0,1.276595744680851,0.9249910934231593
1.0084210526315789,1.276595744680851,0.9244002307514165
1.016842105263158,1.276595744680851,0.9238100424636286
1.0252631578947369,1.276595744680851,0.9232204722511597
1.0336842105263158,1.276595744680851,0.9226315021369373
1.0421052631578946,1.276595744680851,0.922042727470398
1.0505263157894738,1.276595744680851,0.9214553833007812
1.0589473684210526,1.276595744680851,0.9208687259833823
1.0673684210526315,1.276595744680851,0.9202824086023611
1.0757894736842104,1.276595744680851,0.9501010948333715
1.0,1.3085106382978722,0.9250377098469471
1.0084210526315789,1.3085106382978722,0.9244475839504958
1.016842105263158,1.3085106382978722,0.9238581467643598
1.0252631578947369,1.3085106382978722,0.9232693626972832
1.0336842105263158,1.3085106382978722,0.9226812177321335
1.0421052631578946,1.3085106382978722,0.9220935644116253
1.0505263157894738,1.3085106382978722,0.9215068859266466
1.0589473684210526,1.3085106382978722,0.9209206353698391
1.0673684210526315,1.3085106382978722,0.9625569543859456
1.0,1.3404255319148934,0.9250842783094413
1.0084210526315789,1.3404255319148934,0.9244948585692327
1.016842105263158,1.3404255319148934,0.9239062478454798
1.0252631578947369,1.3404255319148934,0.9233181654590226
1.0336842105263158,1.3404255319148934,0.9227307732217014
1.0421052631578946,1.3404255319148934,0.9221439361281227
1.0505263157894738,1.3404255319148934,0.921557960008613
1.0589473684210526,1.3404255319148934,0.9727126565658182
1.0,1.3723404255319147,0.9251307472004555
1.0084210526315789,1.3723404255319147,0.9245421891182559
1.016842105263158,1.3723404255319147,0.9239541923598154
1.0252631578947369,1.3723404255319147,0.9233665466272214
1.0336842105263158,1.3723404255319147,0.9227802998784682
1.0421052631578946,1.3723404255319147,0.9221942785661668
1.0505263157894738,1.3723404255319147,0.9806160405332776
1.0,1.404255319148936,0.9251772180841726
1.0084210526315789,1.404255319148936,0.9245893882043674
1.016842105263158,1.404255319148936,0.9240022301682984
1.0252631578947369,1.404255319148936,0.9234155695303343
1.0336842105263158,1.404255319148936,0.9228297539521009
1.0421052631578946,1.404255319148936,0.9863180670517977
1.0,1.4361702127659572,0.9252235615831523
1.0084210526315789,1.4361702127659572,0.9246364852988336
1.016842105263158,1.4361702127659572,0.9240500013384008
1.0252631578947369,1.4361702127659572,0.9234642642923063
1.0336842105263158,1.4361702127659572,0.9898727164827505
1.0,1.4680851063829785,0.9252698981717913
1.0084210526315789,1.4680851063829785,0.9246835718240618
1.016842105263158,1.4680851063829785,0.9240976125001907
1.0252631578947369,1.4680851063829785,0.9913367672152162
1.0,1.4999999999999998,0.9253160948719596
1.0084210526315789,1.4999999999999998,0.9247305250110003
1.016842105263158,1.4999999999999998,0.990769625656867


==> data/nesterov_fast_gradient_method/automatic_lyapunov.tex <==
x,y
1,0.16666667576282643
2,0.08987136903089006
3,0.05762905639879118
4,0.04055411290794191
5,0.030272645763642976
6,0.02354732479945501
7,0.018883851566368397
8,0.015506121790061153
9,0.01297530894324322
10,0.01102681620665324
11,0.009492771598590239
12,0.008262224255137623
13,0.007259311064116421
14,0.006430643896869779
15,0.005737729480187643
16,0.005152216550745099
17,0.0046528342013679004
18,0.0042233581708532265
19,0.003851257534841719
20,0.003526642942996314
21,0.0032417320244137503
22,0.0029902655994197766
23,0.002767176792251482
24,0.002568327164350524
25,0.0023903106498802205
26,0.0022303001780142034
27,0.0020859368726091087
28,0.001955225408072277
29,0.0018364984147968319
30,0.0017283260210499076
31,0.0016294897223471235
32,0.0015389397697323421
33,0.0014557713611629897
34,0.00137920112537871
35,0.0013085456977966372
36,0.00124320997552445
37,0.0011826687464833036
38,0.0011264646326032627
39,0.0010741926506427067
40,0.0010254915944919423
41,0.0009800406435396703
42,0.0009375585473822188
43,0.0008977940272131188
44,0.0008605102659543054
45,0.0008255079274688528
46,0.0007926061296542528
47,0.0007616403596894497
48,0.0007324619170987508
49,0.0007049342608948091
50,0.0006789355829169289
51,0.0006543542329230107
52,0.0006310864891190464
53,0.0006090415136811723
54,0.0005881371877061574
55,0.0005682903790008043
56,0.0005494349388247254
57,0.0005315034093463201
58,0.0005144367854757703
59,0.0004981804010890891
60,0.00048268418888623824
61,0.0004679023651180616
62,0.00045379019591840685
63,0.00044030894632415157
64,0.00042742110077005337
65,0.00041508871080878204
66,0.00040328406125029483
67,0.00039207390431681777
68,0.0003812411423944244
69,0.0003708521318207596
70,0.00036088382046465877
71,0.00035131191771580085
72,0.0003421187106727013
73,0.0003332808488310485
74,0.0003247814335799188
75,0.0003166033259271323
76,0.00030873002045560125
77,0.00030114543988185024
78,0.000293841330736007
79,0.00028679799802955596
80,0.00028000363635802874
81,0.0002734495614843716
82,0.00026712508830525726
83,0.0002610154742541971
84,0.00025511669353287837
85,0.0002494084882405545
86,0.0002438962179460878
87,0.0002385628248389896
88,0.000233403005603781
89,0.00022841120205041818
90,0.0002235752888334183
91,0.00021889317218664115
92,0.00021435606090278484
93,0.00020995857652369125
94,0.0002056951935602505
95,0.00020155791520550746
96,0.00019754182441148913
97,0.00019363947042883397
98,0.00018985053770643223
99,0.0001861777675502882
100,0.00018260029637195006


==> data/nesterov_fast_gradient_method/nesterov_first_bound.tex <==
x,y
1,0.2222222222222222
2,0.125
3,0.08
4,0.05555555555555555
5,0.04081632653061224
6,0.03125
7,0.024691358024691357
8,0.02
9,0.01652892561983471
10,0.013888888888888888
11,0.011834319526627219
12,0.01020408163265306
13,0.008888888888888889
14,0.0078125
15,0.006920415224913495
16,0.006172839506172839
17,0.00554016620498615
18,0.005
19,0.0045351473922902496
20,0.004132231404958678
21,0.003780718336483932
22,0.003472222222222222
23,0.0032
24,0.0029585798816568047
25,0.0027434842249657062
26,0.002551020408163265
27,0.0023781212841854932
28,0.0022222222222222222
29,0.002081165452653486
30,0.001953125
31,0.0018365472910927456
32,0.0017301038062283738
33,0.0016326530612244899
34,0.0015432098765432098
35,0.0014609203798392988
36,0.0013850415512465374
37,0.0013149243918474688
38,0.00125
39,0.001189767995240928
40,0.0011337868480725624
41,0.001081665765278529
42,0.0010330578512396695
43,0.0009876543209876543
44,0.000945179584120983
45,0.0009053870529651426
46,0.0008680555555555555
47,0.0008329862557267805
48,0.0008
49,0.0007689350249903883
50,0.0007396449704142012
51,0.000711997152011392
52,0.0006858710562414266
53,0.0006611570247933885
54,0.0006377551020408163
55,0.0006155740227762388
56,0.0005945303210463733
57,0.0005745475438092502
58,0.0005555555555555556
59,0.0005374899220639613
60,0.0005202913631633715
61,0.0005039052658100278
62,0.00048828125
63,0.00047337278106508875
64,0.0004591368227731864
65,0.00044553352639786146
66,0.00043252595155709344
67,0.0004200798151648813
68,0.00040816326530612246
69,0.00039674667724657806
70,0.00038580246913580245
71,0.0003753049352598987
72,0.0003652300949598247
73,0.00035555555555555557
74,0.00034626038781163435
75,0.00033732501264968796
76,0.0003287310979618672
77,0.0003204614645088928
78,0.0003125
79,0.00030483158055174517
80,0.000297441998810232
81,0.00029031789809841774
82,0.0002834467120181406
83,0.0002768166089965398
84,0.00027041644131963225
85,0.0002642356982428326
86,0.00025826446280991736
87,0.0002524933720489837
88,0.0002469135802469136
89,0.00024151672503320854
90,0.00023629489603024575
91,0.00023124060585038732
92,0.00022634676324128565
93,0.00022160664819944597
94,0.00021701388888888888
95,0.0002125624402168137
96,0.00020824656393169514
97,0.00020406081012141618
98,0.0002
99,0.00019605920988138416
100,0.00019223375624759708


==> data/nesterov_fast_gradient_method/nesterov_second_bound.tex <==
x,y
1,0.19098300562505258
2,0.10391637813627973
3,0.0661257368537568
4,0.04605649508558456
5,0.034039462715867656
6,0.026241330100390405
7,0.020878976538332948
8,0.017026126289798604
9,0.014160796056052284
10,0.011969779121984318
11,0.01025550722070044
12,0.008888162156641514
13,0.007779491453952131
14,0.006867746567696076
15,0.0061086420154655395
16,0.005469727829367442
17,0.004926775025659082
18,0.004461389573628299
19,0.004059398870628315
20,0.0037097369934197635
21,0.0034036596510170435
22,0.003134181716143937
23,0.002895667897138157
24,0.002683530602847095
25,0.002494004023209569
26,0.0023239731819384222
27,0.0021708431637677554
28,0.0020324380599003734
29,0.0019069221444694762
30,0.0017927378548274464
31,0.0016885565967198028
32,0.0015932394261542829
33,0.0015058054018331245
34,0.0014254059419807417
35,0.0013513039162600868
36,0.0012828564979062791
37,0.0012195010215873489
38,0.001160743258831708
39,0.00110614764938573
40,0.001055329123825155
41,0.0010079462275720647
42,0.0009636953146023832
43,0.0009223056245782532
44,0.0008835350928866883
45,0.0008471667713430458
46,0.0008130057598082575
47,0.0007808765669498845
48,0.0007506208328245828
49,0.0007220953576231621
50,0.0006951703903784332
51,0.0006697281391406305
52,0.000645661470427063
53,0.0006228727709278415
54,0.0006012729487159122
55,0.0005807805547398101
56,0.0005613210083090139
57,0.0005428259127244136
58,0.0005252324492484741
59,0.0005084828393223032
60,0.0004925238663775969
61,0.0004773064498070868
62,0.0004627852646857758
63,0.00044891840170809965
64,0.00043566706254877393
65,0.0004229952864885558
66,0.0004108697046878682
67,0.000399259318955618
68,0.0003881353022595689
69,0.0003774708185682863
70,0.00036724085991129914
71,0.0003574220988007054
72,0.0003479927543798608
73,0.0003389324708579697
74,0.00033022220695752335
75,0.00032184413524812683
76,0.0003137815503683287
77,0.00030601878524914394
78,0.0002985411345512334
79,0.00029133478461400124
80,0.0002843867492907926
81,0.00027768481111127514
82,0.0002712174672711248
83,0.0002649738800013279
84,0.00025894383091561076
85,0.00025311767897546935
86,0.00024748632174863717
87,0.00024204115966916574
88,0.00023677406303607734
89,0.00023167734151321851
90,0.0002267437159158502
91,0.00022196629208999307
92,0.00021733853670887233
93,0.00021285425482723042
94,0.00020850756904900887
95,0.00020429290017713546
96,0.0002002049492260515
97,0.00019623868068832732
98,0.00019238930695636853
99,0.00018865227380892547
100,0.0001850232468799855


==> data/sublinear_chambolle_pock/chambolle_pock_fixed_point_residual_h0_alpha0.tex <==
x,y
1.0,0.1276595744680851
1.0084210526315789,0.1276595744680851
1.016842105263158,0.1276595744680851
1.0252631578947369,0.1276595744680851
1.0336842105263158,0.1276595744680851
1.0421052631578946,0.1276595744680851
1.0505263157894738,0.1276595744680851
1.0589473684210526,0.1276595744680851
1.0673684210526315,0.1276595744680851
1.0,0.15957446808510636
1.0084210526315789,0.15957446808510636
1.016842105263158,0.15957446808510636
1.0252631578947369,0.15957446808510636
1.0336842105263158,0.15957446808510636
1.0421052631578946,0.15957446808510636
1.0505263157894738,0.15957446808510636
1.0589473684210526,0.15957446808510636
1.0673684210526315,0.15957446808510636
1.0757894736842104,0.15957446808510636
1.0842105263157895,0.15957446808510636
1.0926315789473684,0.15957446808510636
1.1010526315789473,0.15957446808510636
1.1094736842105264,0.15957446808510636
1.1178947368421053,0.15957446808510636
1.1263157894736842,0.15957446808510636
1.134736842105263,0.15957446808510636
1.1431578947368422,0.15957446808510636
1.151578947368421,0.15957446808510636
1.16,0.15957446808510636
1.168421052631579,0.15957446808510636
1.176842105263158,0.15957446808510636
1.1852631578947368,0.15957446808510636
1.1936842105263157,0.15957446808510636
1.0,0.19148936170212766
1.0084210526315789,0.19148936170212766
1.016842105263158,0.19148936170212766
1.0252631578947369,0.19148936170212766
1.0336842105263158,0.19148936170212766
1.0421052631578946,0.19148936170212766
1.0505263157894738,0.19148936170212766
1.0589473684210526,0.19148936170212766
1.0673684210526315,0.19148936170212766
1.0757894736842104,0.19148936170212766
1.0842105263157895,0.19148936170212766
1.0926315789473684,0.19148936170212766
1.1010526315789473,0.19148936170212766
1.1094736842105264,0.19148936170212766
1.1178947368421053,0.19148936170212766
1.1263157894736842,0.19148936170212766
1.134736842105263,0.19148936170212766
1.1431578947368422,0.19148936170212766
1.151578947368421,0.19148936170212766
1.16,0.19148936170212766
1.168421052631579,0.19148936170212766
1.176842105263158,0.19148936170212766
1.1852631578947368,0.19148936170212766
1.1936842105263157,0.19148936170212766
1.2021052631578948,0.19148936170212766
1.2105263157894737,0.19148936170212766
1.2189473684210526,0.19148936170212766
1.2273684210526317,0.19148936170212766
1.2357894736842105,0.19148936170212766
1.2442105263157894,0.19148936170212766
1.2526315789473683,0.19148936170212766
1.2610526315789474,0.19148936170212766
1.2694736842105263,0.19148936170212766
1.2778947368421052,0.19148936170212766
1.2863157894736843,0.19148936170212766
1.2947368421052632,0.19148936170212766
1.0,0.22340425531914893
1.0084210526315789,0.22340425531914893
1.016842105263158,0.22340425531914893
1.0252631578947369,0.22340425531914893
1.0336842105263158,0.22340425531914893
1.0421052631578946,0.22340425531914893
1.0505263157894738,0.22340425531914893
1.0589473684210526,0.22340425531914893
1.0673684210526315,0.22340425531914893
1.0757894736842104,0.22340425531914893
1.0842105263157895,0.22340425531914893
1.0926315789473684,0.22340425531914893
1.1010526315789473,0.22340425531914893
1.1094736842105264,0.22340425531914893
1.1178947368421053,0.22340425531914893
1.1263157894736842,0.22340425531914893
1.134736842105263,0.22340425531914893
1.1431578947368422,0.22340425531914893
1.151578947368421,0.22340425531914893
1.16,0.22340425531914893
1.168421052631579,0.22340425531914893
1.176842105263158,0.22340425531914893
1.1852631578947368,0.22340425531914893
1.1936842105263157,0.22340425531914893
1.2021052631578948,0.22340425531914893
1.2105263157894737,0.22340425531914893
1.2189473684210526,0.22340425531914893
1.2273684210526317,0.22340425531914893
1.2357894736842105,0.22340425531914893
1.2442105263157894,0.22340425531914893
1.2526315789473683,0.22340425531914893
1.2610526315789474,0.22340425531914893
1.2694736842105263,0.22340425531914893
1.2778947368421052,0.22340425531914893
1.2863157894736843,0.22340425531914893
1.2947368421052632,0.22340425531914893
1.303157894736842,0.22340425531914893
1.311578947368421,0.22340425531914893
1.32,0.22340425531914893
1.328421052631579,0.22340425531914893
1.3368421052631578,0.22340425531914893
1.345263157894737,0.22340425531914893
1.3536842105263158,0.22340425531914893
1.3621052631578947,0.22340425531914893
1.3705263157894736,0.22340425531914893
1.3789473684210527,0.22340425531914893
1.0,0.2553191489361702
1.0084210526315789,0.2553191489361702
1.016842105263158,0.2553191489361702
1.0252631578947369,0.2553191489361702
1.0336842105263158,0.2553191489361702
1.0421052631578946,0.2553191489361702
1.0505263157894738,0.2553191489361702
1.0589473684210526,0.2553191489361702
1.0673684210526315,0.2553191489361702
1.0757894736842104,0.2553191489361702
1.0842105263157895,0.2553191489361702
1.0926315789473684,0.2553191489361702
1.1010526315789473,0.2553191489361702
1.1094736842105264,0.2553191489361702
1.1178947368421053,0.2553191489361702
1.1263157894736842,0.2553191489361702
1.134736842105263,0.2553191489361702
1.1431578947368422,0.2553191489361702
1.151578947368421,0.2553191489361702
1.16,0.2553191489361702
1.168421052631579,0.2553191489361702
1.176842105263158,0.2553191489361702
1.1852631578947368,0.2553191489361702
1.1936842105263157,0.2553191489361702
1.2021052631578948,0.2553191489361702
1.2105263157894737,0.2553191489361702
1.2189473684210526,0.2553191489361702
1.2273684210526317,0.2553191489361702
1.2357894736842105,0.2553191489361702
1.2442105263157894,0.2553191489361702
1.2526315789473683,0.2553191489361702
1.2610526315789474,0.2553191489361702
1.2694736842105263,0.2553191489361702
1.2778947368421052,0.2553191489361702
1.2863157894736843,0.2553191489361702
1.2947368421052632,0.2553191489361702
1.303157894736842,0.2553191489361702
1.311578947368421,0.2553191489361702
1.32,0.2553191489361702
1.328421052631579,0.2553191489361702
1.3368421052631578,0.2553191489361702
1.345263157894737,0.2553191489361702
1.3536842105263158,0.2553191489361702
1.3621052631578947,0.2553191489361702
1.3705263157894736,0.2553191489361702
1.3789473684210527,0.2553191489361702
1.3873684210526316,0.2553191489361702
1.3957894736842105,0.2553191489361702
1.4042105263157896,0.2553191489361702
1.4126315789473685,0.2553191489361702
1.4210526315789473,0.2553191489361702
1.4294736842105262,0.2553191489361702
1.0,0.28723404255319146
1.0084210526315789,0.28723404255319146
1.016842105263158,0.28723404255319146
1.0252631578947369,0.28723404255319146
1.0336842105263158,0.28723404255319146
1.0421052631578946,0.28723404255319146
1.0505263157894738,0.28723404255319146
1.0589473684210526,0.28723404255319146
1.0673684210526315,0.28723404255319146
1.0757894736842104,0.28723404255319146
1.0842105263157895,0.28723404255319146
1.0926315789473684,0.28723404255319146
1.1010526315789473,0.28723404255319146
1.1094736842105264,0.28723404255319146
1.1178947368421053,0.28723404255319146
1.1263157894736842,0.28723404255319146
1.134736842105263,0.28723404255319146
1.1431578947368422,0.28723404255319146
1.151578947368421,0.28723404255319146
1.16,0.28723404255319146
1.168421052631579,0.28723404255319146
1.176842105263158,0.28723404255319146
1.1852631578947368,0.28723404255319146
1.1936842105263157,0.28723404255319146
1.2021052631578948,0.28723404255319146
1.2105263157894737,0.28723404255319146
1.2189473684210526,0.28723404255319146
1.2273684210526317,0.28723404255319146
1.2357894736842105,0.28723404255319146
1.2442105263157894,0.28723404255319146
1.2526315789473683,0.28723404255319146
1.2610526315789474,0.28723404255319146
1.2694736842105263,0.28723404255319146
1.2778947368421052,0.28723404255319146
1.2863157894736843,0.28723404255319146
1.2947368421052632,0.28723404255319146
1.303157894736842,0.28723404255319146
1.311578947368421,0.28723404255319146
1.32,0.28723404255319146
1.328421052631579,0.28723404255319146
1.3368421052631578,0.28723404255319146
1.345263157894737,0.28723404255319146
1.3536842105263158,0.28723404255319146
1.3621052631578947,0.28723404255319146
1.3705263157894736,0.28723404255319146
1.3789473684210527,0.28723404255319146
1.3873684210526316,0.28723404255319146
1.3957894736842105,0.28723404255319146
1.4042105263157896,0.28723404255319146
1.4126315789473685,0.28723404255319146
1.4210526315789473,0.28723404255319146
1.4294736842105262,0.28723404255319146
1.4378947368421051,0.28723404255319146
1.4463157894736842,0.28723404255319146
1.454736842105263,0.28723404255319146
1.4631578947368422,0.28723404255319146
1.471578947368421,0.28723404255319146
1.48,0.28723404255319146
1.0,0.3191489361702127
1.0084210526315789,0.3191489361702127
1.016842105263158,0.3191489361702127
1.0252631578947369,0.3191489361702127
1.0336842105263158,0.3191489361702127
1.0421052631578946,0.3191489361702127
1.0505263157894738,0.3191489361702127
1.0589473684210526,0.3191489361702127
1.0673684210526315,0.3191489361702127
1.0757894736842104,0.3191489361702127
1.0842105263157895,0.3191489361702127
1.0926315789473684,0.3191489361702127
1.1010526315789473,0.3191489361702127
1.1094736842105264,0.3191489361702127
1.1178947368421053,0.3191489361702127
1.1263157894736842,0.3191489361702127
1.134736842105263,0.3191489361702127
1.1431578947368422,0.3191489361702127
1.151578947368421,0.3191489361702127
1.16,0.3191489361702127
1.168421052631579,0.3191489361702127
1.176842105263158,0.3191489361702127
1.1852631578947368,0.3191489361702127
1.1936842105263157,0.3191489361702127
1.2021052631578948,0.3191489361702127
1.2105263157894737,0.3191489361702127
1.2189473684210526,0.3191489361702127
1.2273684210526317,0.3191489361702127
1.2357894736842105,0.3191489361702127
1.2442105263157894,0.3191489361702127
1.2526315789473683,0.3191489361702127
1.2610526315789474,0.3191489361702127
1.2694736842105263,0.3191489361702127
1.2778947368421052,0.3191489361702127
1.2863157894736843,0.3191489361702127
1.2947368421052632,0.3191489361702127
1.303157894736842,0.3191489361702127
1.311578947368421,0.3191489361702127
1.32,0.3191489361702127
1.328421052631579,0.3191489361702127
1.3368421052631578,0.3191489361702127
1.345263157894737,0.3191489361702127
1.3536842105263158,0.3191489361702127
1.3621052631578947,0.3191489361702127
1.3705263157894736,0.3191489361702127
1.3789473684210527,0.3191489361702127
1.3873684210526316,0.3191489361702127
1.3957894736842105,0.3191489361702127
1.4042105263157896,0.3191489361702127
1.4126315789473685,0.3191489361702127
1.4210526315789473,0.3191489361702127
1.4294736842105262,0.3191489361702127
1.4378947368421051,0.3191489361702127
1.4463157894736842,0.3191489361702127
1.454736842105263,0.3191489361702127
1.4631578947368422,0.3191489361702127
1.471578947368421,0.3191489361702127
1.48,0.3191489361702127
1.4884210526315789,0.3191489361702127
1.4968421052631578,0.3191489361702127
1.0,0.351063829787234
1.0084210526315789,0.351063829787234
1.016842105263158,0.351063829787234
1.0252631578947369,0.351063829787234
1.0336842105263158,0.351063829787234
1.0421052631578946,0.351063829787234
1.0505263157894738,0.351063829787234
1.0589473684210526,0.351063829787234
1.0673684210526315,0.351063829787234
1.0757894736842104,0.351063829787234
1.0842105263157895,0.351063829787234
1.0926315789473684,0.351063829787234
1.1010526315789473,0.351063829787234
1.1094736842105264,0.351063829787234
1.1178947368421053,0.351063829787234
1.1263157894736842,0.351063829787234
1.134736842105263,0.351063829787234
1.1431578947368422,0.351063829787234
1.151578947368421,0.351063829787234
1.16,0.351063829787234
1.168421052631579,0.351063829787234
1.176842105263158,0.351063829787234
1.1852631578947368,0.351063829787234
1.1936842105263157,0.351063829787234
1.2021052631578948,0.351063829787234
1.2105263157894737,0.351063829787234
1.2189473684210526,0.351063829787234
1.2273684210526317,0.351063829787234
1.2357894736842105,0.351063829787234
1.2442105263157894,0.351063829787234
1.2526315789473683,0.351063829787234
1.2610526315789474,0.351063829787234
1.2694736842105263,0.351063829787234
1.2778947368421052,0.351063829787234
1.2863157894736843,0.351063829787234
1.2947368421052632,0.351063829787234
1.303157894736842,0.351063829787234
1.311578947368421,0.351063829787234
1.32,0.351063829787234
1.328421052631579,0.351063829787234
1.3368421052631578,0.351063829787234
1.345263157894737,0.351063829787234
1.3536842105263158,0.351063829787234
1.3621052631578947,0.351063829787234
1.3705263157894736,0.351063829787234
1.3789473684210527,0.351063829787234
1.3873684210526316,0.351063829787234
1.3957894736842105,0.351063829787234
1.4042105263157896,0.351063829787234
1.4126315789473685,0.351063829787234
1.4210526315789473,0.351063829787234
1.4294736842105262,0.351063829787234
1.4378947368421051,0.351063829787234
1.4463157894736842,0.351063829787234
1.454736842105263,0.351063829787234
1.4631578947368422,0.351063829787234
1.471578947368421,0.351063829787234
1.48,0.351063829787234
1.4884210526315789,0.351063829787234
1.4968421052631578,0.351063829787234
1.5052631578947369,0.351063829787234
1.0,0.3829787234042553
1.0084210526315789,0.3829787234042553
1.016842105263158,0.3829787234042553
1.0252631578947369,0.3829787234042553
1.0336842105263158,0.3829787234042553
1.0421052631578946,0.3829787234042553
1.0505263157894738,0.3829787234042553
1.0589473684210526,0.3829787234042553
1.0673684210526315,0.3829787234042553
1.0757894736842104,0.3829787234042553
1.0842105263157895,0.3829787234042553
1.0926315789473684,0.3829787234042553
1.1010526315789473,0.3829787234042553
1.1094736842105264,0.3829787234042553
1.1178947368421053,0.3829787234042553
1.1263157894736842,0.3829787234042553
1.134736842105263,0.3829787234042553
1.1431578947368422,0.3829787234042553
1.151578947368421,0.3829787234042553
1.16,0.3829787234042553
1.168421052631579,0.3829787234042553
1.176842105263158,0.3829787234042553
1.1852631578947368,0.3829787234042553
1.1936842105263157,0.3829787234042553
1.2021052631578948,0.3829787234042553
1.2105263157894737,0.3829787234042553
1.2189473684210526,0.3829787234042553
1.2273684210526317,0.3829787234042553
1.2357894736842105,0.3829787234042553
1.2442105263157894,0.3829787234042553
1.2526315789473683,0.3829787234042553
1.2610526315789474,0.3829787234042553
1.2694736842105263,0.3829787234042553
1.2778947368421052,0.3829787234042553
1.2863157894736843,0.3829787234042553
1.2947368421052632,0.3829787234042553
1.303157894736842,0.3829787234042553
1.311578947368421,0.3829787234042553
1.32,0.3829787234042553
1.328421052631579,0.3829787234042553
1.3368421052631578,0.3829787234042553
1.345263157894737,0.3829787234042553
1.3536842105263158,0.3829787234042553
1.3621052631578947,0.3829787234042553
1.3705263157894736,0.3829787234042553
1.3789473684210527,0.3829787234042553
1.3873684210526316,0.3829787234042553
1.3957894736842105,0.3829787234042553
1.4042105263157896,0.3829787234042553
1.4126315789473685,0.3829787234042553
1.4210526315789473,0.3829787234042553
1.4294736842105262,0.3829787234042553
1.4378947368421051,0.3829787234042553
1.4463157894736842,0.3829787234042553
1.454736842105263,0.3829787234042553
1.4631578947368422,0.3829787234042553
1.471578947368421,0.3829787234042553
1.48,0.3829787234042553
1.4884210526315789,0.3829787234042553
1.0,0.4148936170212766
1.0084210526315789,0.4148936170212766
1.016842105263158,0.4148936170212766
1.0252631578947369,0.4148936170212766
1.0336842105263158,0.4148936170212766
1.0421052631578946,0.4148936170212766
1.0505263157894738,0.4148936170212766
1.0589473684210526,0.4148936170212766
1.0673684210526315,0.4148936170212766
1.0757894736842104,0.4148936170212766
1.0842105263157895,0.4148936170212766
1.0926315789473684,0.4148936170212766
1.1010526315789473,0.4148936170212766
1.1094736842105264,0.4148936170212766
1.1178947368421053,0.4148936170212766
1.1263157894736842,0.4148936170212766
1.134736842105263,0.4148936170212766
1.1431578947368422,0.4148936170212766
1.151578947368421,0.4148936170212766
1.16,0.4148936170212766
1.168421052631579,0.4148936170212766
1.176842105263158,0.4148936170212766
1.1852631578947368,0.4148936170212766
1.1936842105263157,0.4148936170212766
1.2021052631578948,0.4148936170212766
1.2105263157894737,0.4148936170212766
1.2189473684210526,0.4148936170212766
1.2273684210526317,0.4148936170212766
1.2357894736842105,0.4148936170212766
1.2442105263157894,0.4148936170212766
1.2526315789473683,0.4148936170212766
1.2610526315789474,0.4148936170212766
1.2694736842105263,0.4148936170212766
1.2778947368421052,0.4148936170212766
1.2863157894736843,0.4148936170212766
1.2947368421052632,0.4148936170212766
1.303157894736842,0.4148936170212766
1.311578947368421,0.4148936170212766
1.32,0.4148936170212766
1.328421052631579,0.4148936170212766
1.3368421052631578,0.4148936170212766
1.345263157894737,0.4148936170212766
1.3536842105263158,0.4148936170212766
1.3621052631578947,0.4148936170212766
1.3705263157894736,0.4148936170212766
1.3789473684210527,0.4148936170212766
1.3873684210526316,0.4148936170212766
1.3957894736842105,0.4148936170212766
1.4042105263157896,0.4148936170212766
1.4126315789473685,0.4148936170212766
1.4210526315789473,0.4148936170212766
1.4294736842105262,0.4148936170212766
1.4378947368421051,0.4148936170212766
1.4463157894736842,0.4148936170212766
1.454736842105263,0.4148936170212766
1.4631578947368422,0.4148936170212766
1.471578947368421,0.4148936170212766
1.0,0.44680851063829785
1.0084210526315789,0.44680851063829785
1.016842105263158,0.44680851063829785
1.0252631578947369,0.44680851063829785
1.0336842105263158,0.44680851063829785
1.0421052631578946,0.44680851063829785
1.0505263157894738,0.44680851063829785
1.0589473684210526,0.44680851063829785
1.0673684210526315,0.44680851063829785
1.0757894736842104,0.44680851063829785
1.0842105263157895,0.44680851063829785
1.0926315789473684,0.44680851063829785
1.1010526315789473,0.44680851063829785
1.1094736842105264,0.44680851063829785
1.1178947368421053,0.44680851063829785
1.1263157894736842,0.44680851063829785
1.134736842105263,0.44680851063829785
1.1431578947368422,0.44680851063829785
1.151578947368421,0.44680851063829785
1.16,0.44680851063829785
1.168421052631579,0.44680851063829785
1.176842105263158,0.44680851063829785
1.1852631578947368,0.44680851063829785
1.1936842105263157,0.44680851063829785
1.2021052631578948,0.44680851063829785
1.2105263157894737,0.44680851063829785
1.2189473684210526,0.44680851063829785
1.2273684210526317,0.44680851063829785
1.2357894736842105,0.44680851063829785
1.2442105263157894,0.44680851063829785
1.2526315789473683,0.44680851063829785
1.2610526315789474,0.44680851063829785
1.2694736842105263,0.44680851063829785
1.2778947368421052,0.44680851063829785
1.2863157894736843,0.44680851063829785
1.2947368421052632,0.44680851063829785
1.303157894736842,0.44680851063829785
1.311578947368421,0.44680851063829785
1.32,0.44680851063829785
1.328421052631579,0.44680851063829785
1.3368421052631578,0.44680851063829785
1.345263157894737,0.44680851063829785
1.3536842105263158,0.44680851063829785
1.3621052631578947,0.44680851063829785
1.3705263157894736,0.44680851063829785
1.3789473684210527,0.44680851063829785
1.3873684210526316,0.44680851063829785
1.3957894736842105,0.44680851063829785
1.4042105263157896,0.44680851063829785
1.4126315789473685,0.44680851063829785
1.4210526315789473,0.44680851063829785
1.4294736842105262,0.44680851063829785
1.4378947368421051,0.44680851063829785
1.4463157894736842,0.44680851063829785
1.0,0.4787234042553191
1.0084210526315789,0.4787234042553191
1.016842105263158,0.4787234042553191
1.0252631578947369,0.4787234042553191
1.0336842105263158,0.4787234042553191
1.0421052631578946,0.4787234042553191
1.0505263157894738,0.4787234042553191
1.0589473684210526,0.4787234042553191
1.0673684210526315,0.4787234042553191
1.0757894736842104,0.4787234042553191
1.0842105263157895,0.4787234042553191
1.0926315789473684,0.4787234042553191
1.1010526315789473,0.4787234042553191
1.1094736842105264,0.4787234042553191
1.1178947368421053,0.4787234042553191
1.1263157894736842,0.4787234042553191
1.134736842105263,0.4787234042553191
1.1431578947368422,0.4787234042553191
1.151578947368421,0.4787234042553191
1.16,0.4787234042553191
1.168421052631579,0.4787234042553191
1.176842105263158,0.4787234042553191
1.1852631578947368,0.4787234042553191
1.1936842105263157,0.4787234042553191
1.2021052631578948,0.4787234042553191
1.2105263157894737,0.4787234042553191
1.2189473684210526,0.4787234042553191
1.2273684210526317,0.4787234042553191
1.2357894736842105,0.4787234042553191
1.2442105263157894,0.4787234042553191
1.2526315789473683,0.4787234042553191
1.2610526315789474,0.4787234042553191
1.2694736842105263,0.4787234042553191
1.2778947368421052,0.4787234042553191
1.2863157894736843,0.4787234042553191
1.2947368421052632,0.4787234042553191
1.303157894736842,0.4787234042553191
1.311578947368421,0.4787234042553191
1.32,0.4787234042553191
1.328421052631579,0.4787234042553191
1.3368421052631578,0.4787234042553191
1.345263157894737,0.4787234042553191
1.3536842105263158,0.4787234042553191
1.3621052631578947,0.4787234042553191
1.3705263157894736,0.4787234042553191
1.3789473684210527,0.4787234042553191
1.3873684210526316,0.4787234042553191
1.3957894736842105,0.4787234042553191
1.4042105263157896,0.4787234042553191
1.4126315789473685,0.4787234042553191
1.4210526315789473,0.4787234042553191
1.4294736842105262,0.4787234042553191
1.0,0.5106382978723404
1.0084210526315789,0.5106382978723404
1.016842105263158,0.5106382978723404
1.0252631578947369,0.5106382978723404
1.0336842105263158,0.5106382978723404
1.0421052631578946,0.5106382978723404
1.0505263157894738,0.5106382978723404
1.0589473684210526,0.5106382978723404
1.0673684210526315,0.5106382978723404
1.0757894736842104,0.5106382978723404
1.0842105263157895,0.5106382978723404
1.0926315789473684,0.5106382978723404
1.1010526315789473,0.5106382978723404
1.1094736842105264,0.5106382978723404
1.1178947368421053,0.5106382978723404
1.1263157894736842,0.5106382978723404
1.134736842105263,0.5106382978723404
1.1431578947368422,0.5106382978723404
1.151578947368421,0.5106382978723404
1.16,0.5106382978723404
1.168421052631579,0.5106382978723404
1.176842105263158,0.5106382978723404
1.1852631578947368,0.5106382978723404
1.1936842105263157,0.5106382978723404
1.2021052631578948,0.5106382978723404
1.2105263157894737,0.5106382978723404
1.2189473684210526,0.5106382978723404
1.2273684210526317,0.5106382978723404
1.2357894736842105,0.5106382978723404
1.2442105263157894,0.5106382978723404
1.2526315789473683,0.5106382978723404
1.2610526315789474,0.5106382978723404
1.2694736842105263,0.5106382978723404
1.2778947368421052,0.5106382978723404
1.2863157894736843,0.5106382978723404
1.2947368421052632,0.5106382978723404
1.303157894736842,0.5106382978723404
1.311578947368421,0.5106382978723404
1.32,0.5106382978723404
1.328421052631579,0.5106382978723404
1.3368421052631578,0.5106382978723404
1.345263157894737,0.5106382978723404
1.3536842105263158,0.5106382978723404
1.3621052631578947,0.5106382978723404
1.3705263157894736,0.5106382978723404
1.3789473684210527,0.5106382978723404
1.3873684210526316,0.5106382978723404
1.3957894736842105,0.5106382978723404
1.4042105263157896,0.5106382978723404
1.0,0.5425531914893617
1.0084210526315789,0.5425531914893617
1.016842105263158,0.5425531914893617
1.0252631578947369,0.5425531914893617
1.0336842105263158,0.5425531914893617
1.0421052631578946,0.5425531914893617
1.0505263157894738,0.5425531914893617
1.0589473684210526,0.5425531914893617
1.0673684210526315,0.5425531914893617
1.0757894736842104,0.5425531914893617
1.0842105263157895,0.5425531914893617
1.0926315789473684,0.5425531914893617
1.1010526315789473,0.5425531914893617
1.1094736842105264,0.5425531914893617
1.1178947368421053,0.5425531914893617
1.1263157894736842,0.5425531914893617
1.134736842105263,0.5425531914893617
1.1431578947368422,0.5425531914893617
1.151578947368421,0.5425531914893617
1.16,0.5425531914893617
1.168421052631579,0.5425531914893617
1.176842105263158,0.5425531914893617
1.1852631578947368,0.5425531914893617
1.1936842105263157,0.5425531914893617
1.2021052631578948,0.5425531914893617
1.2105263157894737,0.5425531914893617
1.2189473684210526,0.5425531914893617
1.2273684210526317,0.5425531914893617
1.2357894736842105,0.5425531914893617
1.2442105263157894,0.5425531914893617
1.2526315789473683,0.5425531914893617
1.2610526315789474,0.5425531914893617
1.2694736842105263,0.5425531914893617
1.2778947368421052,0.5425531914893617
1.2863157894736843,0.5425531914893617
1.2947368421052632,0.5425531914893617
1.303157894736842,0.5425531914893617
1.311578947368421,0.5425531914893617
1.32,0.5425531914893617
1.328421052631579,0.5425531914893617
1.3368421052631578,0.5425531914893617
1.345263157894737,0.5425531914893617
1.3536842105263158,0.5425531914893617
1.3621052631578947,0.5425531914893617
1.3705263157894736,0.5425531914893617
1.3789473684210527,0.5425531914893617
1.0,0.5744680851063829
1.0084210526315789,0.5744680851063829
1.016842105263158,0.5744680851063829
1.0252631578947369,0.5744680851063829
1.0336842105263158,0.5744680851063829
1.0421052631578946,0.5744680851063829
1.0505263157894738,0.5744680851063829
1.0589473684210526,0.5744680851063829
1.0673684210526315,0.5744680851063829
1.0757894736842104,0.5744680851063829
1.0842105263157895,0.5744680851063829
1.0926315789473684,0.5744680851063829
1.1010526315789473,0.5744680851063829
1.1094736842105264,0.5744680851063829
1.1178947368421053,0.5744680851063829
1.1263157894736842,0.5744680851063829
1.134736842105263,0.5744680851063829
1.1431578947368422,0.5744680851063829
1.151578947368421,0.5744680851063829
1.16,0.5744680851063829
1.168421052631579,0.5744680851063829
1.176842105263158,0.5744680851063829
1.1852631578947368,0.5744680851063829
1.1936842105263157,0.5744680851063829
1.2021052631578948,0.5744680851063829
1.2105263157894737,0.5744680851063829
1.2189473684210526,0.5744680851063829
1.2273684210526317,0.5744680851063829
1.2357894736842105,0.5744680851063829
1.2442105263157894,0.5744680851063829
1.2526315789473683,0.5744680851063829
1.2610526315789474,0.5744680851063829
1.2694736842105263,0.5744680851063829
1.2778947368421052,0.5744680851063829
1.2863157894736843,0.5744680851063829
1.2947368421052632,0.5744680851063829
1.303157894736842,0.5744680851063829
1.311578947368421,0.5744680851063829
1.32,0.5744680851063829
1.328421052631579,0.5744680851063829
1.3368421052631578,0.5744680851063829
1.345263157894737,0.5744680851063829
1.3536842105263158,0.5744680851063829
1.3621052631578947,0.5744680851063829
1.0,0.6063829787234042
1.0084210526315789,0.6063829787234042
1.016842105263158,0.6063829787234042
1.0252631578947369,0.6063829787234042
1.0336842105263158,0.6063829787234042
1.0421052631578946,0.6063829787234042
1.0505263157894738,0.6063829787234042
1.0589473684210526,0.6063829787234042
1.0673684210526315,0.6063829787234042
1.0757894736842104,0.6063829787234042
1.0842105263157895,0.6063829787234042
1.0926315789473684,0.6063829787234042
1.1010526315789473,0.6063829787234042
1.1094736842105264,0.6063829787234042
1.1178947368421053,0.6063829787234042
1.1263157894736842,0.6063829787234042
1.134736842105263,0.6063829787234042
1.1431578947368422,0.6063829787234042
1.151578947368421,0.6063829787234042
1.16,0.6063829787234042
1.168421052631579,0.6063829787234042
1.176842105263158,0.6063829787234042
1.1852631578947368,0.6063829787234042
1.1936842105263157,0.6063829787234042
1.2021052631578948,0.6063829787234042
1.2105263157894737,0.6063829787234042
1.2189473684210526,0.6063829787234042
1.2273684210526317,0.6063829787234042
1.2357894736842105,0.6063829787234042
1.2442105263157894,0.6063829787234042
1.2526315789473683,0.6063829787234042
1.2610526315789474,0.6063829787234042
1.2694736842105263,0.6063829787234042
1.2778947368421052,0.6063829787234042
1.2863157894736843,0.6063829787234042
1.2947368421052632,0.6063829787234042
1.303157894736842,0.6063829787234042
1.311578947368421,0.6063829787234042
1.32,0.6063829787234042
1.328421052631579,0.6063829787234042
1.3368421052631578,0.6063829787234042
1.0,0.6382978723404255
1.0084210526315789,0.6382978723404255
1.016842105263158,0.6382978723404255
1.0252631578947369,0.6382978723404255
1.0336842105263158,0.6382978723404255
1.0421052631578946,0.6382978723404255
1.0505263157894738,0.6382978723404255
1.0589473684210526,0.6382978723404255
1.0673684210526315,0.6382978723404255
1.0757894736842104,0.6382978723404255
1.0842105263157895,0.6382978723404255
1.0926315789473684,0.6382978723404255
1.1010526315789473,0.6382978723404255
1.1094736842105264,0.6382978723404255
1.1178947368421053,0.6382978723404255
1.1263157894736842,0.6382978723404255
1.134736842105263,0.6382978723404255
1.1431578947368422,0.6382978723404255
1.151578947368421,0.6382978723404255
1.16,0.6382978723404255
1.168421052631579,0.6382978723404255
1.176842105263158,0.6382978723404255
1.1852631578947368,0.6382978723404255
1.1936842105263157,0.6382978723404255
1.2021052631578948,0.6382978723404255
1.2105263157894737,0.6382978723404255
1.2189473684210526,0.6382978723404255
1.2273684210526317,0.6382978723404255
1.2357894736842105,0.6382978723404255
1.2442105263157894,0.6382978723404255
1.2526315789473683,0.6382978723404255
1.2610526315789474,0.6382978723404255
1.2694736842105263,0.6382978723404255
1.2778947368421052,0.6382978723404255
1.2863157894736843,0.6382978723404255
1.2947368421052632,0.6382978723404255
1.303157894736842,0.6382978723404255
1.311578947368421,0.6382978723404255
1.32,0.6382978723404255
1.0,0.6702127659574467
1.0084210526315789,0.6702127659574467
1.016842105263158,0.6702127659574467
1.0252631578947369,0.6702127659574467
1.0336842105263158,0.6702127659574467
1.0421052631578946,0.6702127659574467
1.0505263157894738,0.6702127659574467
1.0589473684210526,0.6702127659574467
1.0673684210526315,0.6702127659574467
1.0757894736842104,0.6702127659574467
1.0842105263157895,0.6702127659574467
1.0926315789473684,0.6702127659574467
1.1010526315789473,0.6702127659574467
1.1094736842105264,0.6702127659574467
1.1178947368421053,0.6702127659574467
1.1263157894736842,0.6702127659574467
1.134736842105263,0.6702127659574467
1.1431578947368422,0.6702127659574467
1.151578947368421,0.6702127659574467
1.16,0.6702127659574467
1.168421052631579,0.6702127659574467
1.176842105263158,0.6702127659574467
1.1852631578947368,0.6702127659574467
1.1936842105263157,0.6702127659574467
1.2021052631578948,0.6702127659574467
1.2105263157894737,0.6702127659574467
1.2189473684210526,0.6702127659574467
1.2273684210526317,0.6702127659574467
1.2357894736842105,0.6702127659574467
1.2442105263157894,0.6702127659574467
1.2526315789473683,0.6702127659574467
1.2610526315789474,0.6702127659574467
1.2694736842105263,0.6702127659574467
1.2778947368421052,0.6702127659574467
1.2863157894736843,0.6702127659574467
1.2947368421052632,0.6702127659574467
1.303157894736842,0.6702127659574467
1.0,0.702127659574468
1.0084210526315789,0.702127659574468
1.016842105263158,0.702127659574468
1.0252631578947369,0.702127659574468
1.0336842105263158,0.702127659574468
1.0421052631578946,0.702127659574468
1.0505263157894738,0.702127659574468
1.0589473684210526,0.702127659574468
1.0673684210526315,0.702127659574468
1.0757894736842104,0.702127659574468
1.0842105263157895,0.702127659574468
1.0926315789473684,0.702127659574468
1.1010526315789473,0.702127659574468
1.1094736842105264,0.702127659574468
1.1178947368421053,0.702127659574468
1.1263157894736842,0.702127659574468
1.134736842105263,0.702127659574468
1.1431578947368422,0.702127659574468
1.151578947368421,0.702127659574468
1.16,0.702127659574468
1.168421052631579,0.702127659574468
1.176842105263158,0.702127659574468
1.1852631578947368,0.702127659574468
1.1936842105263157,0.702127659574468
1.2021052631578948,0.702127659574468
1.2105263157894737,0.702127659574468
1.2189473684210526,0.702127659574468
1.2273684210526317,0.702127659574468
1.2357894736842105,0.702127659574468
1.2442105263157894,0.702127659574468
1.2526315789473683,0.702127659574468
1.2610526315789474,0.702127659574468
1.2694736842105263,0.702127659574468
1.2778947368421052,0.702127659574468
1.2863157894736843,0.702127659574468
1.0,0.7340425531914893
1.0084210526315789,0.7340425531914893
1.016842105263158,0.7340425531914893
1.0252631578947369,0.7340425531914893
1.0336842105263158,0.7340425531914893
1.0421052631578946,0.7340425531914893
1.0505263157894738,0.7340425531914893
1.0589473684210526,0.7340425531914893
1.0673684210526315,0.7340425531914893
1.0757894736842104,0.7340425531914893
1.0842105263157895,0.7340425531914893
1.0926315789473684,0.7340425531914893
1.1010526315789473,0.7340425531914893
1.1094736842105264,0.7340425531914893
1.1178947368421053,0.7340425531914893
1.1263157894736842,0.7340425531914893
1.134736842105263,0.7340425531914893
1.1431578947368422,0.7340425531914893
1.151578947368421,0.7340425531914893
1.16,0.7340425531914893
1.168421052631579,0.7340425531914893
1.176842105263158,0.7340425531914893
1.1852631578947368,0.7340425531914893
1.1936842105263157,0.7340425531914893
1.2021052631578948,0.7340425531914893
1.2105263157894737,0.7340425531914893
1.2189473684210526,0.7340425531914893
1.2273684210526317,0.7340425531914893
1.2357894736842105,0.7340425531914893
1.2442105263157894,0.7340425531914893
1.2526315789473683,0.7340425531914893
1.2610526315789474,0.7340425531914893
1.2694736842105263,0.7340425531914893
1.0,0.7659574468085106
1.0084210526315789,0.7659574468085106
1.016842105263158,0.7659574468085106
1.0252631578947369,0.7659574468085106
1.0336842105263158,0.7659574468085106
1.0421052631578946,0.7659574468085106
1.0505263157894738,0.7659574468085106
1.0589473684210526,0.7659574468085106
1.0673684210526315,0.7659574468085106
1.0757894736842104,0.7659574468085106
1.0842105263157895,0.7659574468085106
1.0926315789473684,0.7659574468085106
1.1010526315789473,0.7659574468085106
1.1094736842105264,0.7659574468085106
1.1178947368421053,0.7659574468085106
1.1263157894736842,0.7659574468085106
1.134736842105263,0.7659574468085106
1.1431578947368422,0.7659574468085106
1.151578947368421,0.7659574468085106
1.16,0.7659574468085106
1.168421052631579,0.7659574468085106
1.176842105263158,0.7659574468085106
1.1852631578947368,0.7659574468085106
1.1936842105263157,0.7659574468085106
1.2021052631578948,0.7659574468085106
1.2105263157894737,0.7659574468085106
1.2189473684210526,0.7659574468085106
1.2273684210526317,0.7659574468085106
1.2357894736842105,0.7659574468085106
1.2442105263157894,0.7659574468085106
1.2526315789473683,0.7659574468085106
1.0,0.7978723404255319
1.0084210526315789,0.7978723404255319
1.016842105263158,0.7978723404255319
1.0252631578947369,0.7978723404255319
1.0336842105263158,0.7978723404255319
1.0421052631578946,0.7978723404255319
1.0505263157894738,0.7978723404255319
1.0589473684210526,0.7978723404255319
1.0673684210526315,0.7978723404255319
1.0757894736842104,0.7978723404255319
1.0842105263157895,0.7978723404255319
1.0926315789473684,0.7978723404255319
1.1010526315789473,0.7978723404255319
1.1094736842105264,0.7978723404255319
1.1178947368421053,0.7978723404255319
1.1263157894736842,0.7978723404255319
1.134736842105263,0.7978723404255319
1.1431578947368422,0.7978723404255319
1.151578947368421,0.7978723404255319
1.16,0.7978723404255319
1.168421052631579,0.7978723404255319
1.176842105263158,0.7978723404255319
1.1852631578947368,0.7978723404255319
1.1936842105263157,0.7978723404255319
1.2021052631578948,0.7978723404255319
1.2105263157894737,0.7978723404255319
1.2189473684210526,0.7978723404255319
1.2273684210526317,0.7978723404255319
1.2357894736842105,0.7978723404255319
1.0,0.8297872340425532
1.0084210526315789,0.8297872340425532
1.016842105263158,0.8297872340425532
1.0252631578947369,0.8297872340425532
1.0336842105263158,0.8297872340425532
1.0421052631578946,0.8297872340425532
1.0505263157894738,0.8297872340425532
1.0589473684210526,0.8297872340425532
1.0673684210526315,0.8297872340425532
1.0757894736842104,0.8297872340425532
1.0842105263157895,0.8297872340425532
1.0926315789473684,0.8297872340425532
1.1010526315789473,0.8297872340425532
1.1094736842105264,0.8297872340425532
1.1178947368421053,0.8297872340425532
1.1263157894736842,0.8297872340425532
1.134736842105263,0.8297872340425532
1.1431578947368422,0.8297872340425532
1.151578947368421,0.8297872340425532
1.16,0.8297872340425532
1.168421052631579,0.8297872340425532
1.176842105263158,0.8297872340425532
1.1852631578947368,0.8297872340425532
1.1936842105263157,0.8297872340425532
1.2021052631578948,0.8297872340425532
1.2105263157894737,0.8297872340425532
1.2189473684210526,0.8297872340425532
1.0,0.8617021276595744
1.0084210526315789,0.8617021276595744
1.016842105263158,0.8617021276595744
1.0252631578947369,0.8617021276595744
1.0336842105263158,0.8617021276595744
1.0421052631578946,0.8617021276595744
1.0505263157894738,0.8617021276595744
1.0589473684210526,0.8617021276595744
1.0673684210526315,0.8617021276595744
1.0757894736842104,0.8617021276595744
1.0842105263157895,0.8617021276595744
1.0926315789473684,0.8617021276595744
1.1010526315789473,0.8617021276595744
1.1094736842105264,0.8617021276595744
1.1178947368421053,0.8617021276595744
1.1263157894736842,0.8617021276595744
1.134736842105263,0.8617021276595744
1.1431578947368422,0.8617021276595744
1.151578947368421,0.8617021276595744
1.16,0.8617021276595744
1.168421052631579,0.8617021276595744
1.176842105263158,0.8617021276595744
1.1852631578947368,0.8617021276595744
1.1936842105263157,0.8617021276595744
1.2021052631578948,0.8617021276595744
1.2105263157894737,0.8617021276595744
1.0,0.8936170212765957
1.0084210526315789,0.8936170212765957
1.016842105263158,0.8936170212765957
1.0252631578947369,0.8936170212765957
1.0336842105263158,0.8936170212765957
1.0421052631578946,0.8936170212765957
1.0505263157894738,0.8936170212765957
1.0589473684210526,0.8936170212765957
1.0673684210526315,0.8936170212765957
1.0757894736842104,0.8936170212765957
1.0842105263157895,0.8936170212765957
1.0926315789473684,0.8936170212765957
1.1010526315789473,0.8936170212765957
1.1094736842105264,0.8936170212765957
1.1178947368421053,0.8936170212765957
1.1263157894736842,0.8936170212765957
1.134736842105263,0.8936170212765957
1.1431578947368422,0.8936170212765957
1.151578947368421,0.8936170212765957
1.16,0.8936170212765957
1.168421052631579,0.8936170212765957
1.176842105263158,0.8936170212765957
1.1852631578947368,0.8936170212765957
1.1936842105263157,0.8936170212765957
1.0,0.925531914893617
1.0084210526315789,0.925531914893617
1.016842105263158,0.925531914893617
1.0252631578947369,0.925531914893617
1.0336842105263158,0.925531914893617
1.0421052631578946,0.925531914893617
1.0505263157894738,0.925531914893617
1.0589473684210526,0.925531914893617
1.0673684210526315,0.925531914893617
1.0757894736842104,0.925531914893617
1.0842105263157895,0.925531914893617
1.0926315789473684,0.925531914893617
1.1010526315789473,0.925531914893617
1.1094736842105264,0.925531914893617
1.1178947368421053,0.925531914893617
1.1263157894736842,0.925531914893617
1.134736842105263,0.925531914893617
1.1431578947368422,0.925531914893617
1.151578947368421,0.925531914893617
1.16,0.925531914893617
1.168421052631579,0.925531914893617
1.176842105263158,0.925531914893617
1.0,0.9574468085106382
1.0084210526315789,0.9574468085106382
1.016842105263158,0.9574468085106382
1.0252631578947369,0.9574468085106382
1.0336842105263158,0.9574468085106382
1.0421052631578946,0.9574468085106382
1.0505263157894738,0.9574468085106382
1.0589473684210526,0.9574468085106382
1.0673684210526315,0.9574468085106382
1.0757894736842104,0.9574468085106382
1.0842105263157895,0.9574468085106382
1.0926315789473684,0.9574468085106382
1.1010526315789473,0.9574468085106382
1.1094736842105264,0.9574468085106382
1.1178947368421053,0.9574468085106382
1.1263157894736842,0.9574468085106382
1.134736842105263,0.9574468085106382
1.1431578947368422,0.9574468085106382
1.151578947368421,0.9574468085106382
1.16,0.9574468085106382
1.168421052631579,0.9574468085106382
1.0,0.9893617021276595
1.0084210526315789,0.9893617021276595
1.016842105263158,0.9893617021276595
1.0252631578947369,0.9893617021276595
1.0336842105263158,0.9893617021276595
1.0421052631578946,0.9893617021276595
1.0505263157894738,0.9893617021276595
1.0589473684210526,0.9893617021276595
1.0673684210526315,0.9893617021276595
1.0757894736842104,0.9893617021276595
1.0842105263157895,0.9893617021276595
1.0926315789473684,0.9893617021276595
1.1010526315789473,0.9893617021276595
1.1094736842105264,0.9893617021276595
1.1178947368421053,0.9893617021276595
1.1263157894736842,0.9893617021276595
1.134736842105263,0.9893617021276595
1.1431578947368422,0.9893617021276595
1.151578947368421,0.9893617021276595
1.0,1.0212765957446808
1.0084210526315789,1.0212765957446808
1.016842105263158,1.0212765957446808
1.0252631578947369,1.0212765957446808
1.0336842105263158,1.0212765957446808
1.0421052631578946,1.0212765957446808
1.0505263157894738,1.0212765957446808
1.0589473684210526,1.0212765957446808
1.0673684210526315,1.0212765957446808
1.0757894736842104,1.0212765957446808
1.0842105263157895,1.0212765957446808
1.0926315789473684,1.0212765957446808
1.1010526315789473,1.0212765957446808
1.1094736842105264,1.0212765957446808
1.1178947368421053,1.0212765957446808
1.1263157894736842,1.0212765957446808
1.134736842105263,1.0212765957446808
1.1431578947368422,1.0212765957446808
1.0,1.053191489361702
1.0084210526315789,1.053191489361702
1.016842105263158,1.053191489361702
1.0252631578947369,1.053191489361702
1.0336842105263158,1.053191489361702
1.0421052631578946,1.053191489361702
1.0505263157894738,1.053191489361702
1.0589473684210526,1.053191489361702
1.0673684210526315,1.053191489361702
1.0757894736842104,1.053191489361702
1.0842105263157895,1.053191489361702
1.0926315789473684,1.053191489361702
1.1010526315789473,1.053191489361702
1.1094736842105264,1.053191489361702
1.1178947368421053,1.053191489361702
1.1263157894736842,1.053191489361702
1.134736842105263,1.053191489361702
1.0,1.0851063829787233
1.0084210526315789,1.0851063829787233
1.016842105263158,1.0851063829787233
1.0252631578947369,1.0851063829787233
1.0336842105263158,1.0851063829787233
1.0421052631578946,1.0851063829787233
1.0505263157894738,1.0851063829787233
1.0589473684210526,1.0851063829787233
1.0673684210526315,1.0851063829787233
1.0757894736842104,1.0851063829787233
1.0842105263157895,1.0851063829787233
1.0926315789473684,1.0851063829787233
1.1010526315789473,1.0851063829787233
1.1094736842105264,1.0851063829787233
1.1178947368421053,1.0851063829787233
1.0,1.1170212765957446
1.0084210526315789,1.1170212765957446
1.016842105263158,1.1170212765957446
1.0252631578947369,1.1170212765957446
1.0336842105263158,1.1170212765957446
1.0421052631578946,1.1170212765957446
1.0505263157894738,1.1170212765957446
1.0589473684210526,1.1170212765957446
1.0673684210526315,1.1170212765957446
1.0757894736842104,1.1170212765957446
1.0842105263157895,1.1170212765957446
1.0926315789473684,1.1170212765957446
1.1010526315789473,1.1170212765957446
1.1094736842105264,1.1170212765957446
1.0,1.1489361702127658
1.0084210526315789,1.1489361702127658
1.016842105263158,1.1489361702127658
1.0252631578947369,1.1489361702127658
1.0336842105263158,1.1489361702127658
1.0421052631578946,1.1489361702127658
1.0505263157894738,1.1489361702127658
1.0589473684210526,1.1489361702127658
1.0673684210526315,1.1489361702127658
1.0757894736842104,1.1489361702127658
1.0842105263157895,1.1489361702127658
1.0926315789473684,1.1489361702127658
1.1010526315789473,1.1489361702127658
1.0,1.180851063829787
1.0084210526315789,1.180851063829787
1.016842105263158,1.180851063829787
1.0252631578947369,1.180851063829787
1.0336842105263158,1.180851063829787
1.0421052631578946,1.180851063829787
1.0505263157894738,1.180851063829787
1.0589473684210526,1.180851063829787
1.0673684210526315,1.180851063829787
1.0757894736842104,1.180851063829787
1.0842105263157895,1.180851063829787
1.0,1.2127659574468084
1.0084210526315789,1.2127659574468084
1.016842105263158,1.2127659574468084
1.0252631578947369,1.2127659574468084
1.0336842105263158,1.2127659574468084
1.0421052631578946,1.2127659574468084
1.0505263157894738,1.2127659574468084
1.0589473684210526,1.2127659574468084
1.0673684210526315,1.2127659574468084
1.0757894736842104,1.2127659574468084
1.0,1.2446808510638296
1.0084210526315789,1.2446808510638296
1.016842105263158,1.2446808510638296
1.0252631578947369,1.2446808510638296
1.0336842105263158,1.2446808510638296
1.0421052631578946,1.2446808510638296
1.0505263157894738,1.2446808510638296
1.0589473684210526,1.2446808510638296
1.0673684210526315,1.2446808510638296
1.0,1.276595744680851
1.0084210526315789,1.276595744680851
1.016842105263158,1.276595744680851
1.0252631578947369,1.276595744680851
1.0336842105263158,1.276595744680851
1.0421052631578946,1.276595744680851
1.0505263157894738,1.276595744680851
1.0589473684210526,1.276595744680851
1.0,1.3085106382978722
1.0084210526315789,1.3085106382978722
1.016842105263158,1.3085106382978722
1.0252631578947369,1.3085106382978722
1.0336842105263158,1.3085106382978722
1.0421052631578946,1.3085106382978722
1.0505263157894738,1.3085106382978722
1.0,1.3404255319148934
1.0084210526315789,1.3404255319148934
1.016842105263158,1.3404255319148934
1.0252631578947369,1.3404255319148934
1.0336842105263158,1.3404255319148934
1.0421052631578946,1.3404255319148934
1.0,1.3723404255319147
1.0084210526315789,1.3723404255319147
1.016842105263158,1.3723404255319147
1.0252631578947369,1.3723404255319147
1.0,1.404255319148936
1.0084210526315789,1.404255319148936
1.016842105263158,1.404255319148936
1.0,1.4361702127659572
1.0084210526315789,1.4361702127659572
1.0,1.4680851063829785


==> data/sublinear_chambolle_pock/chambolle_pock_fixed_point_residual_h1_alpha0.tex <==
x,y
1.0757894736842104,0.1276595744680851
1.0842105263157895,0.1276595744680851
1.0926315789473684,0.1276595744680851
1.2021052631578948,0.15957446808510636
1.2105263157894737,0.15957446808510636
1.2189473684210526,0.15957446808510636
1.303157894736842,0.19148936170212766
1.311578947368421,0.19148936170212766
1.32,0.19148936170212766
1.328421052631579,0.19148936170212766
1.3873684210526316,0.22340425531914893
1.3957894736842105,0.22340425531914893
1.4042105263157896,0.22340425531914893
1.4126315789473685,0.22340425531914893
1.4210526315789473,0.22340425531914893
1.4294736842105262,0.22340425531914893
1.4378947368421051,0.22340425531914893
1.4378947368421051,0.2553191489361702
1.4463157894736842,0.22340425531914893
1.4463157894736842,0.2553191489361702
1.454736842105263,0.22340425531914893
1.454736842105263,0.2553191489361702
1.4631578947368422,0.22340425531914893
1.4631578947368422,0.2553191489361702
1.471578947368421,0.22340425531914893
1.471578947368421,0.2553191489361702
1.48,0.2553191489361702
1.4884210526315789,0.2553191489361702
1.4884210526315789,0.28723404255319146
1.4968421052631578,0.2553191489361702
1.4968421052631578,0.28723404255319146
1.4968421052631578,0.3829787234042553
1.5052631578947369,0.2553191489361702
1.5052631578947369,0.28723404255319146
1.5052631578947369,0.3191489361702127
1.5136842105263157,0.2553191489361702
1.5136842105263157,0.28723404255319146
1.5136842105263157,0.3191489361702127
1.5136842105263157,0.351063829787234
1.5221052631578948,0.2553191489361702
1.5221052631578948,0.28723404255319146
1.5221052631578948,0.3191489361702127
1.5221052631578948,0.351063829787234
1.5305263157894737,0.2553191489361702
1.5305263157894737,0.28723404255319146
1.5305263157894737,0.3191489361702127
1.5305263157894737,0.351063829787234
1.5389473684210526,0.2553191489361702
1.5389473684210526,0.28723404255319146
1.5389473684210526,0.3191489361702127
1.5473684210526315,0.2553191489361702
1.5473684210526315,0.28723404255319146
1.5473684210526315,0.3191489361702127
1.5557894736842104,0.2553191489361702
1.5557894736842104,0.28723404255319146
1.5557894736842104,0.3191489361702127
1.5642105263157895,0.2553191489361702
1.5642105263157895,0.28723404255319146
1.5726315789473684,0.2553191489361702
1.5726315789473684,0.28723404255319146
1.5810526315789475,0.2553191489361702
1.5810526315789475,0.28723404255319146
1.5894736842105264,0.2553191489361702
1.5894736842105264,0.28723404255319146
1.5978947368421053,0.2553191489361702
1.6063157894736841,0.2553191489361702


==> data/sublinear_chambolle_pock/chambolle_pock_fixed_point_residual_h1_alpha1.tex <==
x,y
1.0,0.06382978723404255
1.0,0.09574468085106383
1.0084210526315789,0.06382978723404255
1.0084210526315789,0.09574468085106383
1.016842105263158,0.06382978723404255
1.016842105263158,0.09574468085106383
1.0252631578947369,0.06382978723404255
1.0252631578947369,0.09574468085106383
1.0336842105263158,0.09574468085106383
1.0421052631578946,0.09574468085106383
1.0505263157894738,0.09574468085106383
1.0589473684210526,0.09574468085106383
1.0673684210526315,0.09574468085106383
1.0757894736842104,0.09574468085106383
1.0842105263157895,0.09574468085106383
1.0926315789473684,0.09574468085106383
1.1010526315789473,0.09574468085106383
1.1010526315789473,0.1276595744680851
1.1094736842105264,0.09574468085106383
1.1094736842105264,0.1276595744680851
1.1178947368421053,0.09574468085106383
1.1178947368421053,0.1276595744680851
1.1263157894736842,0.09574468085106383
1.1263157894736842,0.1276595744680851
1.134736842105263,0.09574468085106383
1.134736842105263,0.1276595744680851
1.1431578947368422,0.09574468085106383
1.1431578947368422,0.1276595744680851
1.151578947368421,0.09574468085106383
1.151578947368421,0.1276595744680851
1.16,0.09574468085106383
1.16,0.1276595744680851
1.168421052631579,0.09574468085106383
1.168421052631579,0.1276595744680851
1.176842105263158,0.09574468085106383
1.176842105263158,0.1276595744680851
1.1852631578947368,0.09574468085106383
1.1852631578947368,0.1276595744680851
1.1936842105263157,0.09574468085106383
1.1936842105263157,0.1276595744680851
1.2021052631578948,0.09574468085106383
1.2021052631578948,0.1276595744680851
1.2105263157894737,0.09574468085106383
1.2105263157894737,0.1276595744680851
1.2189473684210526,0.09574468085106383
1.2189473684210526,0.1276595744680851
1.2273684210526317,0.09574468085106383
1.2273684210526317,0.1276595744680851
1.2273684210526317,0.15957446808510636
1.2357894736842105,0.09574468085106383
1.2357894736842105,0.1276595744680851
1.2357894736842105,0.15957446808510636
1.2442105263157894,0.09574468085106383
1.2442105263157894,0.1276595744680851
1.2442105263157894,0.15957446808510636
1.2526315789473683,0.09574468085106383
1.2526315789473683,0.1276595744680851
1.2526315789473683,0.15957446808510636
1.2610526315789474,0.09574468085106383
1.2610526315789474,0.1276595744680851
1.2610526315789474,0.15957446808510636
1.2694736842105263,0.09574468085106383
1.2694736842105263,0.1276595744680851
1.2694736842105263,0.15957446808510636
1.2778947368421052,0.09574468085106383
1.2778947368421052,0.1276595744680851
1.2778947368421052,0.15957446808510636
1.2863157894736843,0.09574468085106383
1.2863157894736843,0.1276595744680851
1.2863157894736843,0.15957446808510636
1.2863157894736843,0.28723404255319146
1.2947368421052632,0.09574468085106383
1.2947368421052632,0.1276595744680851
1.2947368421052632,0.15957446808510636
1.303157894736842,0.09574468085106383
1.303157894736842,0.1276595744680851
1.303157894736842,0.15957446808510636
1.303157894736842,0.28723404255319146
1.311578947368421,0.09574468085106383
1.311578947368421,0.1276595744680851
1.311578947368421,0.15957446808510636
1.32,0.09574468085106383
1.32,0.1276595744680851
1.32,0.15957446808510636
1.328421052631579,0.09574468085106383
1.328421052631579,0.1276595744680851
1.328421052631579,0.15957446808510636
1.3368421052631578,0.09574468085106383
1.3368421052631578,0.1276595744680851
1.3368421052631578,0.15957446808510636
1.3368421052631578,0.19148936170212766
1.345263157894737,0.09574468085106383
1.345263157894737,0.1276595744680851
1.345263157894737,0.15957446808510636
1.345263157894737,0.19148936170212766
1.3536842105263158,0.09574468085106383
1.3536842105263158,0.1276595744680851
1.3536842105263158,0.15957446808510636
1.3536842105263158,0.19148936170212766
1.3621052631578947,0.09574468085106383
1.3621052631578947,0.1276595744680851
1.3621052631578947,0.15957446808510636
1.3621052631578947,0.19148936170212766
1.3705263157894736,0.09574468085106383
1.3705263157894736,0.1276595744680851
1.3705263157894736,0.15957446808510636
1.3705263157894736,0.19148936170212766
1.3789473684210527,0.09574468085106383
1.3789473684210527,0.1276595744680851
1.3789473684210527,0.15957446808510636
1.3789473684210527,0.19148936170212766
1.3873684210526316,0.09574468085106383
1.3873684210526316,0.1276595744680851
1.3873684210526316,0.15957446808510636
1.3873684210526316,0.19148936170212766
1.3957894736842105,0.09574468085106383
1.3957894736842105,0.1276595744680851
1.3957894736842105,0.15957446808510636
1.3957894736842105,0.19148936170212766
1.4042105263157896,0.09574468085106383
1.4042105263157896,0.1276595744680851
1.4042105263157896,0.15957446808510636
1.4042105263157896,0.19148936170212766
1.4126315789473685,0.1276595744680851
1.4126315789473685,0.15957446808510636
1.4126315789473685,0.19148936170212766
1.4210526315789473,0.1276595744680851
1.4210526315789473,0.15957446808510636
1.4210526315789473,0.19148936170212766
1.4294736842105262,0.1276595744680851
1.4294736842105262,0.15957446808510636
1.4294736842105262,0.19148936170212766
1.4378947368421051,0.1276595744680851
1.4378947368421051,0.15957446808510636
1.4378947368421051,0.19148936170212766
1.4463157894736842,0.1276595744680851
1.4463157894736842,0.15957446808510636
1.4463157894736842,0.19148936170212766
1.454736842105263,0.1276595744680851
1.454736842105263,0.15957446808510636
1.454736842105263,0.19148936170212766
1.4631578947368422,0.1276595744680851
1.4631578947368422,0.15957446808510636
1.4631578947368422,0.19148936170212766
1.471578947368421,0.1276595744680851
1.471578947368421,0.15957446808510636
1.471578947368421,0.19148936170212766
1.48,0.1276595744680851
1.48,0.15957446808510636
1.48,0.19148936170212766
1.48,0.22340425531914893
1.4884210526315789,0.1276595744680851
1.4884210526315789,0.15957446808510636
1.4884210526315789,0.19148936170212766
1.4884210526315789,0.22340425531914893
1.4968421052631578,0.1276595744680851
1.4968421052631578,0.15957446808510636
1.4968421052631578,0.19148936170212766
1.4968421052631578,0.22340425531914893
1.5052631578947369,0.15957446808510636
1.5052631578947369,0.19148936170212766
1.5052631578947369,0.22340425531914893
1.5136842105263157,0.15957446808510636
1.5136842105263157,0.19148936170212766
1.5136842105263157,0.22340425531914893
1.5221052631578948,0.15957446808510636
1.5221052631578948,0.19148936170212766
1.5221052631578948,0.22340425531914893
1.5305263157894737,0.15957446808510636
1.5305263157894737,0.19148936170212766
1.5305263157894737,0.22340425531914893
1.5389473684210526,0.15957446808510636
1.5389473684210526,0.19148936170212766
1.5389473684210526,0.22340425531914893
1.5473684210526315,0.15957446808510636
1.5473684210526315,0.19148936170212766
1.5473684210526315,0.22340425531914893
1.5557894736842104,0.15957446808510636
1.5557894736842104,0.19148936170212766
1.5557894736842104,0.22340425531914893
1.5642105263157895,0.15957446808510636
1.5642105263157895,0.19148936170212766
1.5642105263157895,0.22340425531914893
1.5726315789473684,0.15957446808510636
1.5726315789473684,0.19148936170212766
1.5726315789473684,0.22340425531914893
1.5810526315789475,0.19148936170212766
1.5810526315789475,0.22340425531914893
1.5894736842105264,0.19148936170212766
1.5894736842105264,0.22340425531914893
1.5978947368421053,0.19148936170212766
1.5978947368421053,0.22340425531914893
1.6063157894736841,0.19148936170212766
1.6063157894736841,0.22340425531914893
1.614736842105263,0.19148936170212766
1.614736842105263,0.22340425531914893
1.614736842105263,0.2553191489361702
1.6231578947368421,0.19148936170212766
1.6231578947368421,0.22340425531914893
1.631578947368421,0.19148936170212766
1.631578947368421,0.22340425531914893
1.6400000000000001,0.22340425531914893


==> data/sublinear_chambolle_pock/chambolle_pock_fixed_point_residual_h2_alpha0.tex <==
x,y
1.0,0.031914893617021274
1.0084210526315789,0.031914893617021274
1.016842105263158,0.031914893617021274
1.0252631578947369,0.031914893617021274
1.0336842105263158,0.031914893617021274
1.0336842105263158,0.06382978723404255
1.0421052631578946,0.031914893617021274
1.0421052631578946,0.06382978723404255
1.0505263157894738,0.031914893617021274
1.0505263157894738,0.06382978723404255
1.0589473684210526,0.031914893617021274
1.0589473684210526,0.06382978723404255
1.0673684210526315,0.031914893617021274
1.0673684210526315,0.06382978723404255
1.0757894736842104,0.031914893617021274
1.0757894736842104,0.06382978723404255
1.0842105263157895,0.031914893617021274
1.0842105263157895,0.06382978723404255
1.0926315789473684,0.031914893617021274
1.0926315789473684,0.06382978723404255
1.1010526315789473,0.031914893617021274
1.1010526315789473,0.06382978723404255
1.1010526315789473,1.1489361702127658
1.1094736842105264,0.031914893617021274
1.1094736842105264,0.06382978723404255
1.1178947368421053,0.031914893617021274
1.1178947368421053,0.06382978723404255
1.1263157894736842,0.031914893617021274
1.1263157894736842,0.06382978723404255
1.134736842105263,0.031914893617021274
1.134736842105263,0.06382978723404255
1.134736842105263,1.053191489361702
1.1431578947368422,0.031914893617021274
1.1431578947368422,0.06382978723404255
1.151578947368421,0.031914893617021274
1.151578947368421,0.06382978723404255
1.16,0.031914893617021274
1.16,0.06382978723404255
1.168421052631579,0.031914893617021274
1.168421052631579,0.06382978723404255
1.176842105263158,0.031914893617021274
1.176842105263158,0.06382978723404255
1.1852631578947368,0.031914893617021274
1.1852631578947368,0.06382978723404255
1.1936842105263157,0.031914893617021274
1.1936842105263157,0.06382978723404255
1.2021052631578948,0.031914893617021274
1.2021052631578948,0.06382978723404255
1.2105263157894737,0.031914893617021274
1.2105263157894737,0.06382978723404255
1.2189473684210526,0.031914893617021274
1.2189473684210526,0.06382978723404255
1.2273684210526317,0.031914893617021274
1.2273684210526317,0.06382978723404255
1.2357894736842105,0.031914893617021274
1.2357894736842105,0.06382978723404255
1.2442105263157894,0.031914893617021274
1.2442105263157894,0.06382978723404255
1.2526315789473683,0.031914893617021274
1.2526315789473683,0.06382978723404255
1.2610526315789474,0.031914893617021274
1.2610526315789474,0.06382978723404255
1.2694736842105263,0.031914893617021274
1.2694736842105263,0.06382978723404255
1.2778947368421052,0.031914893617021274
1.2778947368421052,0.06382978723404255
1.2863157894736843,0.031914893617021274
1.2863157894736843,0.06382978723404255
1.2947368421052632,0.031914893617021274
1.2947368421052632,0.06382978723404255
1.303157894736842,0.031914893617021274
1.303157894736842,0.06382978723404255
1.311578947368421,0.031914893617021274
1.311578947368421,0.06382978723404255
1.32,0.031914893617021274
1.32,0.06382978723404255
1.328421052631579,0.031914893617021274
1.328421052631579,0.06382978723404255
1.3368421052631578,0.031914893617021274
1.3368421052631578,0.06382978723404255
1.345263157894737,0.031914893617021274
1.345263157894737,0.06382978723404255
1.3536842105263158,0.031914893617021274
1.3536842105263158,0.06382978723404255
1.3621052631578947,0.031914893617021274
1.3621052631578947,0.06382978723404255
1.3705263157894736,0.031914893617021274
1.3705263157894736,0.06382978723404255
1.3789473684210527,0.031914893617021274
1.3789473684210527,0.06382978723404255
1.3873684210526316,0.031914893617021274
1.3873684210526316,0.06382978723404255
1.3957894736842105,0.031914893617021274
1.3957894736842105,0.06382978723404255
1.4042105263157896,0.031914893617021274
1.4042105263157896,0.06382978723404255
1.4126315789473685,0.031914893617021274
1.4126315789473685,0.06382978723404255
1.4126315789473685,0.09574468085106383
1.4210526315789473,0.031914893617021274
1.4210526315789473,0.06382978723404255
1.4210526315789473,0.09574468085106383
1.4294736842105262,0.031914893617021274
1.4294736842105262,0.06382978723404255
1.4294736842105262,0.09574468085106383
1.4294736842105262,0.4787234042553191
1.4378947368421051,0.031914893617021274
1.4378947368421051,0.06382978723404255
1.4378947368421051,0.09574468085106383
1.4463157894736842,0.031914893617021274
1.4463157894736842,0.06382978723404255
1.4463157894736842,0.09574468085106383
1.454736842105263,0.031914893617021274
1.454736842105263,0.06382978723404255
1.454736842105263,0.09574468085106383
1.4631578947368422,0.031914893617021274
1.4631578947368422,0.06382978723404255
1.4631578947368422,0.09574468085106383
1.471578947368421,0.031914893617021274
1.471578947368421,0.06382978723404255
1.471578947368421,0.09574468085106383
1.48,0.031914893617021274
1.48,0.06382978723404255
1.48,0.09574468085106383
1.4884210526315789,0.031914893617021274
1.4884210526315789,0.06382978723404255
1.4884210526315789,0.09574468085106383
1.4968421052631578,0.031914893617021274
1.4968421052631578,0.06382978723404255
1.4968421052631578,0.09574468085106383
1.5052631578947369,0.031914893617021274
1.5052631578947369,0.06382978723404255
1.5052631578947369,0.09574468085106383
1.5052631578947369,0.1276595744680851
1.5136842105263157,0.031914893617021274
1.5136842105263157,0.06382978723404255
1.5136842105263157,0.09574468085106383
1.5136842105263157,0.1276595744680851
1.5221052631578948,0.031914893617021274
1.5221052631578948,0.06382978723404255
1.5221052631578948,0.09574468085106383
1.5221052631578948,0.1276595744680851
1.5305263157894737,0.031914893617021274
1.5305263157894737,0.06382978723404255
1.5305263157894737,0.09574468085106383
1.5305263157894737,0.1276595744680851
1.5389473684210526,0.031914893617021274
1.5389473684210526,0.06382978723404255
1.5389473684210526,0.09574468085106383
1.5389473684210526,0.1276595744680851
1.5473684210526315,0.031914893617021274
1.5473684210526315,0.06382978723404255
1.5473684210526315,0.09574468085106383
1.5473684210526315,0.1276595744680851
1.5557894736842104,0.031914893617021274
1.5557894736842104,0.06382978723404255
1.5557894736842104,0.09574468085106383
1.5557894736842104,0.1276595744680851
1.5642105263157895,0.031914893617021274
1.5642105263157895,0.06382978723404255
1.5642105263157895,0.09574468085106383
1.5642105263157895,0.1276595744680851
1.5726315789473684,0.031914893617021274
1.5726315789473684,0.06382978723404255
1.5726315789473684,0.09574468085106383
1.5726315789473684,0.1276595744680851
1.5810526315789475,0.031914893617021274
1.5810526315789475,0.06382978723404255
1.5810526315789475,0.09574468085106383
1.5810526315789475,0.1276595744680851
1.5810526315789475,0.15957446808510636
1.5894736842105264,0.031914893617021274
1.5894736842105264,0.06382978723404255
1.5894736842105264,0.09574468085106383
1.5894736842105264,0.1276595744680851
1.5894736842105264,0.15957446808510636
1.5978947368421053,0.031914893617021274
1.5978947368421053,0.06382978723404255
1.5978947368421053,0.09574468085106383
1.5978947368421053,0.1276595744680851
1.5978947368421053,0.15957446808510636
1.6063157894736841,0.031914893617021274
1.6063157894736841,0.06382978723404255
1.6063157894736841,0.09574468085106383
1.6063157894736841,0.1276595744680851
1.6063157894736841,0.15957446808510636
1.614736842105263,0.031914893617021274
1.614736842105263,0.06382978723404255
1.614736842105263,0.09574468085106383
1.614736842105263,0.1276595744680851
1.614736842105263,0.15957446808510636
1.6231578947368421,0.031914893617021274
1.6231578947368421,0.06382978723404255
1.6231578947368421,0.09574468085106383
1.6231578947368421,0.1276595744680851
1.6231578947368421,0.15957446808510636
1.6231578947368421,0.2553191489361702
1.631578947368421,0.031914893617021274
1.631578947368421,0.06382978723404255
1.631578947368421,0.09574468085106383
1.631578947368421,0.1276595744680851
1.631578947368421,0.15957446808510636
1.6400000000000001,0.031914893617021274
1.6400000000000001,0.06382978723404255
1.6400000000000001,0.09574468085106383
1.6400000000000001,0.1276595744680851
1.6400000000000001,0.15957446808510636
1.6400000000000001,0.19148936170212766
1.648421052631579,0.031914893617021274
1.648421052631579,0.06382978723404255
1.648421052631579,0.09574468085106383
1.648421052631579,0.1276595744680851
1.648421052631579,0.15957446808510636
1.648421052631579,0.19148936170212766
1.648421052631579,0.22340425531914893
1.656842105263158,0.06382978723404255
1.656842105263158,0.09574468085106383
1.656842105263158,0.1276595744680851
1.656842105263158,0.15957446808510636
1.656842105263158,0.19148936170212766
1.656842105263158,0.22340425531914893
1.6652631578947368,0.06382978723404255
1.6652631578947368,0.09574468085106383
1.6652631578947368,0.1276595744680851
1.6652631578947368,0.15957446808510636
1.6652631578947368,0.19148936170212766
1.6736842105263157,0.06382978723404255
1.6736842105263157,0.09574468085106383
1.6736842105263157,0.1276595744680851
1.6736842105263157,0.15957446808510636
1.6736842105263157,0.19148936170212766
1.6821052631578948,0.06382978723404255
1.6821052631578948,0.09574468085106383
1.6821052631578948,0.1276595744680851
1.6821052631578948,0.15957446808510636
1.6821052631578948,0.19148936170212766
1.6905263157894737,0.06382978723404255
1.6905263157894737,0.09574468085106383
1.6905263157894737,0.1276595744680851
1.6905263157894737,0.15957446808510636
1.6905263157894737,0.19148936170212766
1.6989473684210528,0.06382978723404255
1.6989473684210528,0.09574468085106383
1.6989473684210528,0.1276595744680851
1.6989473684210528,0.15957446808510636
1.7073684210526316,0.06382978723404255
1.7073684210526316,0.09574468085106383
1.7073684210526316,0.1276595744680851
1.7073684210526316,0.15957446808510636
1.7157894736842105,0.06382978723404255
1.7157894736842105,0.09574468085106383
1.7157894736842105,0.1276595744680851
1.7157894736842105,0.15957446808510636
1.7242105263157894,0.09574468085106383

